Empowering Retrieval-based Conversational Recommendation with Contrasting User Preferences

Conversational recommender systems (CRSs) are designed to suggest the target item that the user is likely to prefer through multi-turn conversations. Recent studies stress that capturing sentiments in user conversations improves recommendation accuracy. However, they employ a single user representation, which may fail to distinguish between contrasting user intentions, such as likes and dislikes, potentially leading to suboptimal performance. To this end, we propose a novel conversational recommender model, called COntrasting user pReference expAnsion and Learning (CORAL). Firstly, CORAL extracts the user's hidden preferences through contrasting preference expansion using the reasoning capacity of the LLMs. Based on the potential preference, CORAL explicitly differentiates the contrasting preferences and leverages them into the recommendation process via preference-aware learning. Extensive experiments show that CORAL significantly outperforms existing methods in three benchmark datasets, improving up to 99.72% in Recall@10. The code and datasets are available at https://github.com/kookeej/CORAL

==> body/WSDM/0_abstract.tex <==
%%
%% The abstract is a short summary of the work to be presented in the
%% article.

\begin{abstract}
% Conversational Recommender Systems(CRSs)는 사용자와 실시간 대화를 통해 사용자가 가장 좋아할 법한 상품을 추천하는 시스템이다.
% Large language models(LLMs)의 괄목할만한 성장과 함께 대부분의 많은 연구들을 LLM을 recommender로써 활용하거나 agent로 활용함으로서 대화형 추천 시스템을 다루려고 하였다.
% 하지만 LLM이 갖는 몇 가지 한계를 개선하기 위해 retriever를 증강하려는 시도들이 있지만, 대부분의 연구는 CRS를 기존의 information retriever(IR)로 취급하여 해결하고 있다. 
% However, simply treating conversations as queries and items as documents, as in traditional IR tasks, is insufficient 왜냐하면 CRS의 dialogue는 multifaceted intention을 갖고 text similarity와 user preference 사이에는 괴리가 존재하기 때문이다. 
% In this paper, 우리는 사용자의 like와 dislike 정보를 명시적으로 구분하고 이를 효과적인 추천에 반영하기 위한 novel framework인 \ours(Like or Dislike: Leveraging Multifaceted User Preference retrieval-Enhanced Conversational Recommendation)을 제안한다.
% By leveraging LLMs to extract implicit user preferences, \ours\,enhances the alignment between these preferences and the retrieval process. 또한, retriever 학습 과정에서 이러한 multifaceted preferences를 명시적으로 반영히기 위한 preference-aware alignment learning 방식을 통해 language model을 user preference similarity를 잘 반영할 수 있도록 하였다. 우리는 광범위한 실험을 통해 실험적으로 제안방법이 기존 learning-based method와 LLM을 outperform함을 확인하였고, 모든 데이터셋에 대해 popularity bias에 강건하여 tail group에서 최대 Recall@1에서 약 550\% 높은 성능을 달성하였음을 실험적으로 입증하였다.

Conversational recommender systems (CRS) are designed to suggest the item that the user might prefer through real-time conversations. With the significant progress in large language models (LLMs), recent studies have explored using LLMs as recommenders or agents in CRS. However, much of the research still utilizes CRS from a traditional information retrieval (IR) perspective, which may not adequately capture the complexity of conversations and the disconnect between text similarity and user preferences. In our paper, we introduce a new method, called \ours, which explicitly differentiates between users' likes and dislikes and integrates this information into the recommendation process. By utilizing LLMs to uncover implicit user preferences, \ours\ enhances the alignment between like/dislike preferences and the retrieval process. Through preference-aware alignment learning, \ours\ ensures that LLMs capture subtle user preference similarities. Extensive experiments show that \ours\ outperforms existing methods and is robust against popularity bias across all datasets.

%Conversational Recommender System (CRS) are designed to suggest items that users might prefer by interacting with them through real-time dialogue. With the significant progress in large language models (LLMs), numerous studies have explored using LLMs as recommenders or agents in CRS. Despite attempts to improve retrievers to address certain shortcomings of LLMs, much of the research continues to view CRS through the lens of traditional information retrieval (IR). However, handling dialogues as queries and items as documents, as done in standard IR, is inadequate since the conversations are complex and reveal a disconnect between text similarity and user preferences.
%In this paper, we propose a novel framework, called \ours, which \emph{explicitly distinguishes between users' like and dislike information} and incorporates it into the recommendation process.
%By utilizing LLMs to extract implicit user preferences, \ours enhances the alignment between these preferences and the retrieval process. Through a preference-aware alignment learning approach during retriever training, \ours ensures that LLMs to capture user preference similarities.
%Extensive experiments demonstrate that \ours outperforms existing methods, while also proving to be robust against popularity bias across all datasets, achieving up to a 550\% improvement in Recall@1 performance for the tail group.


% Recent research on Conversational Recommender Systems (CRSs) using large language models (LLMs) has grown rapidly, but LLMs still face several limitations. Efforts have been made to enhance CRS by improving retrieval capabilities and framing item search from an information retrieval (IR) perspective. However, simply treating conversations as queries and items as documents, as in traditional IR tasks, is insufficient. This is because the text similarity captured by language models fundamentally differs from the multi-preference similarity of users.
% To address these limitations, we propose a novel retrieval model, \ours\,(Like or Dislike), which explicitly integrates user preferences by distinguishing between "likes" and "dislikes," and introduces a new preference-aware alignment training approach that accounts for multiple user preferences. By leveraging LLMs to extract implicit user preferences, \ours\,enhances the alignment between these preferences and the retrieval process. Through extensive experiments on conversational recommendation datasets in both the movie and application domains, \ours\,demonstrates superior performance, particularly in mitigating popularity bias and improving recommendations for less popular items.
\end{abstract}


% Collaborative filtering (CF) plays a critical role in the development of recommender systems. Most CF methods utilize an encoder to embed users and items into the same representation space, and the Bayesian personalized ranking (BPR) loss is usually adopted as the objective function to learn informative encoders. Existing studies mainly focus on designing more powerful encoders (e.g., graph neural network) to learn better representations. However, few efforts have been devoted to investigating the desired properties of representations in CF, which is important to understand the rationale of existing CF methods and design new learning objectives. In this paper, we measure the representation quality in CF from the perspective of alignment and uniformity on the hypersphere. We first theoretically reveal the connection between the BPR loss and these two properties. Then, we empirically analyze the learning dynamics of typical CF methods in terms of quantified alignment and uniformity, which shows that better alignment or uniformity both contribute to higher recommendation performance. Based on the analyses results, a learning objective that directly optimizes these two properties is proposed, named DirectAU. We conduct extensive experiments on three public datasets, and the proposed learning framework with a simple matrix factorization model leads to significant performance improvements compared to state-of-the-art CF methods. Our implementations are publicly available at this https URL.

==> body/WSDM/1_introduction.tex <==
\input{Figures_tex/fig_motivating}

\section{Introduction}
\label{sec:introduction}
% CRS 정의
Conversational recommender systems (CRS) aims to identify user needs through natural language dialogue and subsequently provide optimal recommendations based on this understanding.
In contrast to traditional recommender systems that rely mainly on implicit signals like purchasing patterns or click behavior, CRS facilitates direct user interaction via natural language. This allows users to explicitly communicate their preferences, for instance, by expressing, \textit{"I prefer action films over horror."} This characteristic poses a distinctive challenge for CRS, as it must simultaneously handle natural language processing tasks and deliver precise recommendations.

% 기존의 CRS 연구들은 external knowledge (\eg, knowledge graph)를 결합하여 item과 attribute에 대한 표현력과 이해도를 개선함으로써 reprentation을 풍부하게 표현하는 방법에 집중해 왔다~\cite{crs-kg2019kbrd, crs-kg2020kgsf, crs-kg2024kascrs,crs2021revcore, crs2022mese, crs2022unicrs}.
% 하지만, 이러한 접근은 단순히 발화 내 언급되는 entity나 keyword만 고려하기 때문에 대화의 복잡한 문맥과 사용자의 암묵적인 선호를 충분히 반영하지 못한다.
% 이를 해결하기 위해 item metadata를 활용하거나 ~\cite{crs2022mese}나 item review 검색을 통해 ~\cite{crs2021revcore} 부족한 context information을 보완하려는 연구들이 이루어졌다.
% 최근에는 Large language models(LLMs)이 가진 enormous world knowledge와 contextual reasoning ability는 추천 분야로의 적용을 확산시켰으며, 특히 complex dialogue understanding ability와 fluent generation ability는 CRS 분야의 발전을 가속화하고 있다~\cite{crs-llm2023chatrec,crs-llm2023llmzs,crs-llm2024chatcrs,crs-llm2024interecagent}.
Early CRS studies primarily focused on improving item and attribute representations by incorporating external knowledge sources, such as knowledge graphs, to enhance the expressiveness and understanding of these elements. However, these methods tend to address only the entities or keywords explicitly mentioned in the dialogues, often leading to an insufficient understanding of the nuanced context and users' implicit preferences.
% Several studies have attempted to address the lack of contextual information by utilizing item metadata~\cite{crs2022mese} or incorporating item reviews~\cite{crs2021revcore}. More recently, large-scale language models (LLMs) have been increasingly applied to the recommendation domain due to their vast world knowledge and contextual reasoning capabilities. This has significantly advanced the conversational recommender system (CRS) field by leveraging LLMs' ability to understand and fluently generate complex dialogues~\cite{crs-llm2023chatrec, crs-llm2023llmzs, crs-llm2024chatcrs, crs-llm2024interecagent}.
Several studies have attempted to address the lack of contextual information by leveraging item metadata~\cite{crs2022mese} or incorporating item reviews~\cite{crs2021revcore}. More recently, large language models (LLMs) have been increasingly utilized in the recommendation domain due to their vast world knowledge and contextual reasoning capabilities~\cite{llm-rec2023chatgptgoodsearchinvestigating, llm-rec2023uncoveringchatgpt, crs-llm2024chatgptconversationalrecommendationrefining, llm-rank2024recrankerinstructiontuninglarge, llm-rank2023llamarec}. This has led to significant advancements in the CRS field by harnessing LLMs' ability to comprehend complex dialogues. ~\cite{crs-llm2023chatrec, crs-llm2023llmzs, crs-llm2024chatcrs, crs-llm2024interecagent}.

% 그러나 이러한 진전에도 불구하고, LLM을 recommender로 활용하는 추천 시스템에는 몇 가지 중요한 한계가 드러나고 있다.
% 추천 시스템은 user interaction signal을 기반으로 한 선호 추론이 이루어지는데, 이는 LLM이 사전에 학습한 지식과 다소 상이하다.
% 이로 인해 LLM의 internal knowledge와 reasoning ability는 collaborative signal 포착과 중요한 격차가 존재하며 ~\cite{rs-llm2024alignllm}, 일부 task에서는 전통적인 추천 방법에 비해 낮은 성능을 보일 수 있다~\cite{rs-llm2023chatgptgoodrec}.
% 뿐만 아니라, LLM은 popularity bias으로 인해 반복적으로 인기 있는 항목을 추천하는 경향성이 있으며 out-of-dataset item을 생성하거나 hallucinated recommendation을 생성할 가능성이 있음이 지적되었다 ~\cite{crs-llm2023llmzs}.
% However, despite these advancements, several significant limitations have emerged when using LLMs as recommenders in recommendation systems. Traditional recommendation systems infer user preferences based on interaction signals, which differ from the pre-trained knowledge embedded in LLMs. As a result, there is a significant gap between LLMs' internal knowledge and reasoning capabilities and their ability to capture collaborative filtering signals~\cite{rs-llm2024alignllm}, which can lead to lower performance compared to traditional recommendation methods in certain tasks~\cite{rs-llm2023chatgptgoodrec}. Additionally, LLMs are prone to popularity bias, frequently recommending popular items, and may generate out-of-dataset or hallucinated recommendations~\cite{crs-llm2023llmzs}.

% 이러한 한계를 극복하기 위해 최근에는 언어모델을 item search 관점에서 개선하려는 연구들이 이루어지고 있다~\cite{emb2024bridging, ir-dataset2024AlignLM2IR, crs-ret2023CRSRetbaseline, crs-ret2024nls}.
% ~\cite{crs-ret2023CRSRetbaseline}에서는 BM25를 사용하여 대화를 query로, item을 document로 취급하여 dialogue history가 들어오면 이를 기반으로 사용자가 가장 좋아할 법한 item을 sparse retriever를 통해 찾는 방법을 제안하였으며, 간단하지만 기존 external knowledge에 의존하는 연구들과 비견할만한 성능을 보였다. 
% To overcome these limitations, recent research has focused on improving language models from the perspective of item search~\cite{emb2024bridging, ir-dataset2024AlignLM2IR, crs-ret2023CRSRetbaseline, crs-ret2024nls}. For instance,~\cite{crs-ret2023CRSRetbaseline} proposed a method that uses BM25 to treat dialogues as queries and items as documents. When dialogue history is provided, this approach employs a sparse retriever to identify the items that the user is most likely to prefer based on the dialogue. Despite its simplicity, this method demonstrated performance comparable to existing studies that rely on external knowledge.
Despite advancements, LLMs as recommender face limitations in capturing user preferences, as they rely on pre-trained knowledge rather than interaction signals, leading to gaps in collaborative filtering and lower performance in some tasks~\cite{rs-llm2024alignllm, rs-llm2023chatgptgoodrec}.
Additionally, LLMs often exhibit popularity bias and may produce hallucinated recommendations~\cite{crs-llm2023llmzs}.
To address these issues, recent studies have focused on enhancing LLMs as recommender with item search methods.
Specifically, ~\cite{crs-ret2023CRSRetbaseline} reformulate CRS task to retrieval task, treating dialogues as queries and items as documents.
By employing a sparse retriever to match user preferences, it achieved performance comparable to knowledge-based approaches.

% 하지만, 기존의 information retrieval task처럼 dialogue를 query로 사용하여 item search를 하는 접근은 적절하지 않다.
% 단순히 dialogue와 item metadata 사이의 lexical matching을 통해 아이템을 검색하는 방법은 추천 시스템에서 사용자의 복잡한 선호도를 정확하게 반영하기에는 한계가 있는데, 이는 IR과 CRS 사이의 다음의 차이가 있기 때문이다:


% However, using dialogue as a query for item search, similar to traditional information retrieval tasks, is not an appropriate approach.
% The method of retrieving items based solely on lexical matching between dialogue and item metadata has limitations in accurately reflecting the complex user preferences in a recommendation system.
% This inadequacy arises due to the following key differences between IR and CRS:
However, these methods still have some limitations due to the discrepancy between retrieval and CRS.

% like/dislike가 필요한 이유
% \textbf{(i) 기존 retrieval은 query가 single intention을 가지는 반면, CRS에서는 dialogue에는 사용자의 다면적인 선호가 담겨있다.
% }예를 들어, 사용자는 대화를 통해 표면적인 선호(shallow preferences)뿐만 아니라 item의 feature에 대해 다양한 선호(multifaceted preferences, \eg, like/dislike)를 드러내며, 때로는 명시적으로 표현되지 않은 암묵적인 선호도 존재할 수 있다.
% 예를 들어, like와 dislike를 구분하여 반영하지 않고 retrieve한다면 dialogue에서 사용자가 dislike를 표현한 항목이 포함된 아이템이 의미적 유사도를 기반으로 retrieve될 수 있다. (Fig. 1의 sparse retriever 부분)
\textbf{\textit{Limitation 1.} Traditional retrieval assumes that the query has an atomic intention, whereas in CRS, dialogues encapsulate users' multifaceted preferences.}
% For instance, through conversation, users not only express shallow preferences but also reveal diverse preferences regarding an item's features (\eg, \textit{like/dislike}). Additionally, there may be implicit preferences that are not explicitly stated.
For example, in dialogues, users express a range of preferences for various attributes of an item. (\eg, love, enjoy, hate)
Neglecting this spectrum of preference, items containing features the user has expressed a dislike for could still be retrieved based on semantic similarity alone (as illustrated in the sparse retriever section of Figure~\ref{fig:motivating}).
This highlights the importance of distinguishing and appropriately reflecting the different aspects of user preferences in the retrieval process within CRS.

% 학습을 해야 하는 이유
% \textbf{(ii) 언어모델의 의미적 텍스트 유사성과 사용자 선호 유사성 사이는 차이가 존재한다.
% }Semantic similarity를 반영하는 dense retriever는 aims to find 가장 적절한 document given user query, 그 둘의 의미적 유사도를 가깝게 하는 것에 초점을 맞춘다.
% 하지만 CRS에서 dialogue 내에는 앞서 언급한 것과 같이 다양한 intention이 존재하기 때문에 semantic search를 활용하더라도 CRS에 align되지 않은 retriever는 대화에서 드러나는 preference 정보와 meta 정보 간의 차이를 효과적으로 처리하지 못할 가능성이 크다.
% 즉, Figure 1에서 나타난바와 같이 단순히 lexical matching이나 사용자의 like/dislike preferences를 전혀 고려하지 않고 item search를 하는 것이 아니라, user preference aware search를 한다는 점에서 제안한 preference-aware alignment training의 효과성을 정성적으로 확인할 수 있다.
% 따라서 이를 해결하기 위해서는 item의 meta information이나 user의 dialogue 내의 다양한 preference, 특히 like와 dislike를 고려하는 과정이 필요하며, 언어모델의 semantic similarity와 preference similarity 간의 차이를 줄이기 위한 추가적인 조정과 학습이 필요하다.
\textbf{\textit{Limitation 2.} There is a misalignment between the semantic text similarity and user preference}
Dense retrievers, which prioritize semantic similarity, aim to identify the most relevant documents based on a user's query by emphasizing meaning.
However, CRS requires not only identifying semantic similarity, but also linking the user's preferences to the specific features of the items.
% However, as previously mentioned, CRS frequently involves dialogues with multiple intents. Even when using semantic search, retrievers not specifically designed for CRS may struggle to effectively manage the discrepancies between user preferences expressed in dialogue and the meta-information of the items.

For example, as shown in Figure ~\ref{fig:motivating}, simply relying on a sparse retriever or an untrained dense retriever can lead to wrong answer.
If item searches are conducted without considering the user's preferences or by solely focusing on lexical matching, the recommendation results might not align with the user's true preferences.
Since existing methods fail to integrate preference and semantic similarity effectively, it necessitates the need for training and inference framework that can harmonize both aspects.
% Even when using semantic search, retrievers not specifically designed for CRS may struggle to effectively manage the discrepancies between user preferences expressed in dialogue and the meta-information of the items.
% Therefore, it is crucial to incorporate both the meta-information of the items and the diverse preferences expressed in user dialogues, particularly distinguishing between "likes" and "dislikes." 
% Additionally, further adjustment and training are needed to bridge the gap between the semantic similarity recognized by language models and the preference similarity essential for CRS.


% 이를 해결하기 위해, 본 논문에서는 사용자의 'like'와 'dislike' 정보를 효과적으로 반영할 수 있는 새로운 검색 모델인 \ours을 제안한다. 
% 구체적으로, 우리는 사용자의 explicit/implicit preference를 효과적으로 반영하는 dense retriever를 설계하고 이를 효과적으로 align하는 것을 목표로 한다.
% 먼저 LLM을 통해 대화 내 사용자의 like/dislike 선호와 관련된 explicit/implicit preference를 추출한 후, 이를 retriever 학습에 명시적으로 반영하기 위해 두 가지 핵심 접근을 제안한다:
% (i) Extracting user preferences through LLM: LLM의 뛰어난 reasoning 능력과 지식을 활용하여 대화 내의 표면적인 선호(shallow preference)를 기반으로 사용자의 암시적 선호(implicit preference)를 추출한다. 사용자의 "like"와 "dislike"를 명확하게 구분하여 모델에 반영함으로써 사용자가 선호하는 아이템과 선호하지 않은 아이템을 정교하게 구별할 수 있게 되면 더 나은 개인화된 추천을 제공할 수 있다.
% (ii) Enhancing performance by preference-aware retriever through user-preference alignment: 단순히 텍스트 유사성에 기반한 검색이 아닌, 추출된 사용자 선호 정보를 검색 모델의 학습 과정에 반영함으로써, 사용자의 실제 선호와 일치하는 추천을 제공할 수 있도록 개선한다. 이를 통해 검색 모델과 사용자 선호 간의 불일치를 줄여 맞춤형 추천의 정확도를 높인다.

To address these limitations, we propose a novel retrieval model, \ours, designed to effectively incorporate preferences as shown in figure ~\ref{fig:model_architecture}.
Specifically, our approach focuses on designing a framework that effectively reflects users' explicit and implicit preferences and aims to align these preferences with the items.
Our method involves two key approaches:
\textit{(i) Preference-aware Representation:} First, by leveraging the reasoning capabilities and extensive knowledge of LLMs, we extract users' implicit preferences based on the shallow preferences expressed in dialogues and categorize them into likes and dislikes.
Then, we obtain preference-aware representation, which can be obtained by encoding preferences in addition to the dialogue or metadata.
\textit{(ii) Preference-aware Alignment Training:} Instead of relying solely on text similarity for retrieval, we incorporate the extracted user preference information into the training of the retrieval model.
This learning method directly aligns the user's preferences with the item's features.
This combination of preference extraction and alignment ensures that \ours\ delivers more accurate and personalized search results by effectively capturing and integrating user preferences into the retrieval model.
Our contributions in this paper can be summarized as follows:

% To evaluate \ours, we conduct extensive experiments on conversational recommendation datasets across different domains. Experimental results demonstrate that our method significantly outperforms existing approaches, particularly in mitigating popularity bias and improving recommendations for less popular items. Our contributions in this paper can be summarized as follows:

\begin{itemize}[leftmargin=5mm]
\item We extract user/item preference in two domains, application and movie, and systematically investigate the impact of user preferences in CRS item search.
\item We design a novel framework that explicitly incorporates user preferences into the recommendation, leading to more personalized and effective recommendations.
\item Additionally, we conduct extensive experiments to validate the effectiveness of \ours. Results show that \ours\, effectively mitigating the misalignment between retrieval and CRS.
\end{itemize}

% Our experiments demonstrated that \ours\,outperforms learning-based models, including LLMs, in both the movie and app domains. Although \ours\,showed generally lower performance on the REDIAL dataset compared to LLMs, it proved to be more robust against popularity bias, achieving a 550\% improvement in Recall@1 for unpopular items.

To evaluate \ours, we conduct extensive experiments on conversational recommendation datasets across various domains.
Specifically, \ours\, demonstrates performance comparable to learning-based models, including LLMs, in both the movie and app domains.
Also, our experiment shows that \ours\ is highly effective in mitigating popularity bias, demonstrating a significant advantage over LLMs.


==> body/WSDM/2_related_work.tex <==
\section{Related Work}\label{sec:related_work}
\textbf{Traditional CRS.} 
% 초기 CRS은 주로 \textit{attribute-based approach}를 사용하여 간단한 규칙 기반 시스템이나 사전 정의된 템플릿을 통해 추천을 제공했다~\cite{crs2018saur, crs2020ear}.
% 사용자는 시스템이 제공한 속성 기반 질문(\textit{e.g., Do you like videos for animations?})에 명시적으로 피드백을 제공하여 시스템이 다음 추천을 조정하도록 했다. 이는 사용자가 시스템과 상호작용하는 과정을 통해 점진적으로 더 나은 추천을 제공하려는 초기의 시도를 보여주지만, 미리 정의된 대화 흐름과 템플릿 기반 발화로 인해 깊이 있는 사용자 경험이나 추천 정밀도에서 한계를 가진다. 
% 자연어처리 기술의 발전과 함께, 대화형 추천 시스템은 언어모델 학습을 통해 대화 내 사용자의 의도를 보다 정확히 파악하고 human-like 생성이 가능하게 되었다.
% 제한된 대화에서 user preference를 더 잘 추출하기 위해 external knowledge\textit{(e.g., knowledge graph, reviews, metadata)}를 결합하여 부족한 context information을 보완하는 방법들이 주로 제안되었다~\cite{crs-kg2019kbrd, crs-kg2020kgsf, crs-kg2024kascrs, crs2021revcore, crs2022mese}. 
% 특히, 지식 그래프 기반 모델~\cite{crs-kg2019kbrd, crs-kg2020kgsf, crs-kg2024kascrs}은 지식 그래프를 활용하여 대화 컨텍스트와 사용자 선호도 간의 연결을 강화하였고,
% RevCore~\cite{crs2021revcore}와 MESE~\cite{crs2022mese}는 각각 리뷰 텍스트와 metadata를 사용하여 부족한 context information을 보충하였다. $C^2$-CRS~\cite{crs2023c2crs}는 multi-type external data를 효과적으로 leveraging하는 방법을 탐구하으며, UniCRS~\cite{crs2022unicrs}에서는 기존의 recommendation module과 conversation module를 따로 학습하는 방식은 semantic inconsistency가 존재하기 때문에 이 semantic gap을 prompt learning paradigm을 통해 완화하고자 하였다.
% However, 이러한 연구들은 제한된 대화 내에서 user 또는 item representation quality를 개선하기 위해 external knowledge에 지나치게 의존한다는 한계가 있으며, 대화 내 entity나 keyword만 고려하고 implicit user preference를 반영하기 위해 대화 내의 복잡한 context는 고려하지 못한다는 한계가 있다.
Early conversational recommender systems (CRS) primarily utilized an \textit{attribute-based approach}, offering recommendations through simple rule-based systems or predefined templates~\cite{crs2018saur, crs2020ear}.
Users explicitly provided feedback to attribute-based questions (\textit{e.g., Do you like videos for animations?}) posed by the system, enabling it to adjust subsequent recommendations.
This illustrates an early attempt to incrementally provide better recommendations through user interaction, but it was limited by predefined conversational flows and template-based utterances, leading to shallow user experiences.
% With advancements in natural language processing (NLP), conversational recommender systems have evolved to more accurately discern user intentions within dialogues, enabling human-like generation.
To better extract user preferences from limited dialogues, methods incorporating external knowledge (\textit{e.g., knowledge graphs, reviews, metadata}) have been predominantly proposed to supplement insufficient context information~\cite{crs-kg2019kbrd, crs-kg2020kgsf, crs-kg2024kascrs, crs2021revcore, crs2022mese}.
In particular, knowledge graph-based models~\cite{crs-kg2019kbrd, crs-kg2020kgsf, crs-kg2024kascrs} have utilized knowledge graphs to strengthen the link between conversational context and user preferences.
RevCore~\cite{crs2021revcore} and MESE~\cite{crs2022mese} have employed review texts and metadata, respectively, to augment the lacking context information.
$C^2$-CRS~\cite{crs2023c2crs} explored methods to effectively leverage multi-type external data, and UniCRS~\cite{crs2022unicrs} aimed to mitigate the semantic inconsistency between the traditional recommendation and conversation modules by using the prompt learning paradigm.

However, these studies often rely excessively on external knowledge to improve user or item representation quality within limited dialogues, and can only utilize entities or keywords within the dialogue 
Consequently, they fail to address complex context that reflects implicit user preferences.


\noindent \textbf{CRS with LLM.}
% LLM의 출현은 AI 전반적으로 전례없는 비약적인 발전을 이루었으며, 개인화 추천시스템 분야에서도 사용자에게 필요한 정보를 자연스럽고 설명가능한 형태로 제공할 뿐만 아니라~\cite{rs-llm2023largelanguagemodelsmeet}, rating prediction이나 review summarization과 같은 다양한 추천 task에서 traditional methods와 비견할 만한 성능을 보였다~\cite{rs-llm2023chatgptgoodrec}.
% 이를 CRS에 적용하려는 연구들이 많이 등장하였으며, LLM의 등장은 더 이상 CRS를 수동적인 정보 필터링 매체가 아닌 능동적이고 사용자 참여적인 시스템으로 만들었고~\cite{crs-llm2023chatrec, crs-llm2024chatcrs, crs-llm2024interecagent}, LLM이 가진 방대한 world knowledge와 complex reasoning ability는 기존 knowledge graph와 같은 external knowledge에 의존하던 연구들을 대체할 수 있게 되었다.
% 또한, 기존에는 추천 모듈과 대화 모듈을 따로 학습해야 했지만, LLM의 뛰어난 대화 생성과 추론 능력을 이용하여 추천과 대화의 전환을 효과적으로 통제하고 자연스러운 대화를 생성함으로써 기존의 분리된 두 모듈을 하나의 통합된 모델로 활용할 수 있게 되었다~\cite{crs-llm2023chatrec,crs-llm2024interecagent}.
% 특히 InteRecAgent~\cite{crs-llm2024interecagent}는 기존 도구 계획 과업에서 보여준 LLM의 뛰어난 계획 능력을 활용하여 입력되는 사용자의 발화에 따라 계획하고 도구를 통합 활용하는 에이전트로 활용하여 추천 성능을 개선하였다.
% ~\cite{crs-llm2023llmzs}는 LLM이 영화 추천에서 기존의 학습 기반 모델을 능가할 수 있음을 보여주었으나, 동시에 여전히 LLM이 popularity bias와 out-of-dataset item, hallucinated recommendation 문제가 발생한다는 점이 지적되었다.
The emergence of Large Language Models (LLMs) has led to unprecedented advancements in AI, particularly by enhancing personalized recommendation systems through the provision of essential information in a natural and explainable manner. There has been an increase in attempts to use LLMs not only as ranking models~\cite{llm-rank2023llamarec, llm-rank2024recrankerinstructiontuninglarge} but also as recommendation agents~\cite{agent-rec2023agentcf, agent-rec2024recmind}. Additionally, many studies focus on evaluating the performance of LLMs in recommendation tasks~\cite{rs-llm2023largelanguagemodelsmeet, llm-rec2023uncoveringchatgpt, llm-rec2023chatgptgoodsearchinvestigating}. These models have demonstrated performance comparable to traditional methods in various recommendation tasks such as rating prediction and review summarization~\cite{rs-llm2023chatgptgoodrec}. Numerous studies are exploring the application of LLMs to Conversational Recommender Systems (CRS), transforming CRS from passive information filtering media into active, user-engaging systems~\cite{crs-llm2023chatrec, crs-llm2024chatcrs, crs-llm2024interecagent, crs-llm2023conversationalrecommenderlargelanguage, crs-llm2024musechat, crs-llm2024chatgptconversationalrecommendationrefining, crs-llm2023llmzs}. The extensive world knowledge and complex reasoning abilities of LLMs have the potential to replace studies that rely on external knowledge sources such as knowledge graphs.

However, studies like~\cite{crs-llm2023llmzs} have shown that while LLMs can outperform traditional learning-based models in tasks such as movie recommendations, they also highlight ongoing issues such as popularity bias, out-of-dataset items, and incorrect recommendations.

% Recommender system을 item retrieval task로 재해석하는 연구들이 등장하고 있다\cite{crs-ret2023CRSRetbaseline, crs-ret2024nls, emb2024bridging, rec-ret2024blair}. 특히, CRS에 retriever를 증강함으로써 ~\cite{crs-ret2023CRSRetbaseline, crs-ret2024nls} CRS 문제를 풀려고 하는 연구들이 있고, 특히 dialogue를 query, item을 document로 취급함으로써 BM25를 이용하여 사용자과 가장 관련있는 아이템을 검색하고자 하였다. 몇몇 연구들은 기존의 language model이 item recommendation과 item search task와 align되지 않았음을 지적하며, product embedding을 위한 사전 학습 방식을 제안하거나 ~\cite{rec-ret2024blair}, CRS에서 item search를 위한 language model embedding 학습을 위한 데이터셋을 제안하였다~\cite{ir-dataset2024AlignLM2IR}.

% 본 연구에서는 LLM의 강력한 추론 능력을 사용자 선호도 모델링을 위한 preference information augmentation에 활용한다.
% 특히, 사용자의 like/dislike 선호를 모두 생성하고 이 다면적인 선호를 모두 고려할 수 잇는 참신한 preference-aware alignment 방식을 제안한다.
% 이를 활용하여 검색 모델을 학습함으로써 textual similarity와 preference similarity 사이의 gap을 완화할 수 있을 것이다.
\noindent \textbf{Recommendation as Item Retrieval.} 
Recent studies are reinterpreting recommender systems as item retrieval tasks, introducing innovative methods to enhance Conversational Recommender Systems (CRS) with retrievers~\cite{crs-ret2023CRSRetbaseline, crs-ret2024nls}. Notably, ~\cite{crs-ret2023CRSRetbaseline, crs-ret2024nls} aim to solve CRS challenges by augmenting retrievers, particularly by treating dialogues as queries and items as documents, using BM25~\cite{bm252021pyserini} to search for items most relevant to the user. Some studies have highlighted that traditional language models do not align well with item recommendation and search tasks, proposing pre-training approaches for product embeddings~\cite{rec-ret2024blair} or datasets aimed at training language model embeddings for item search in CRS~\cite{ir-dataset2024AlignLM2IR}.

We leverage the powerful inferencing capabilities of LLMs for modeling user preferences through preference information augmentation. Specifically, we propose a novel preference-aware alignment method that generates and considers both like and dislike preferences of users. By utilizing this approach to train search models, we anticipate mitigating the gap between textual similarity and preference similarity.


==> body/WSDM/3_model.tex <==
\input{Figures_tex/fig_pref_extraction}
\input{Figures_tex/fig_model}
\section{Proposed Model: \ours}\label{sec:Proposed Method}


\subsection{Overall Framework}
\noindent \textbf{Problem definition.}
% $\mathcal{C}$, $\mathcal{U}$, $\mathcal{I}$, $\mathcal{V}$는 각각 Dialogue, 사용자, 아이템, vocabulary의 집합을 의미한다.
Formally, let $\mathcal{C}$ represent the set of dialogue histories, $\mathcal{U}$ the set of users, $\mathcal{I}$ the set of items, and $\mathcal{V}$ the vocabulary set.
% User $u \in \mathcal{U}$의 dialogue $c \in\mathcal{C}$는 $t$ turns의 utterance로 구성되어 있고, $t$-th turn의 utterance는 다음과 같이 구성되어 있다 $(r_t, s_t)_t$.
The dialogue $c \in \mathcal{C}$ for a user $u \in \mathcal{U}$ consists of $t$ turns of utterances. Each utterance at the $t$-th turn is represented as a pair $(r_t, s_t)$, where $r_t$ indicates the role in the conversation, either the user $u$ (denoted as [User]) seeking an item, or the recommender (denoted as [Recommender]) recommending an item or asking a question.
$s_t$, is the utterance itself, $s_t \in \mathcal{V}$, spoken by the respective role $r_t$.
% 또한 item $i\in \mathcal{I}$는 list of textual metadata $m_i = (m_{i,1},...,m_{i,|M|})$를 갖는다 where $|M|$ is the item metadata의 계수.
Additionally, each item $i \in \mathcal{I}$ is associated with a list of textual metadata $m_i = (m_{i,1},...,m_{i,|M|})$, where $|M|$ represents the number of metadata attributes for the item.
% The item $i$의 $j$번째 metadata는 key-value 형태: $m_{i,j} = (k_{i, j}, v_{i, j})$로 표현되어 있다, (\eg key: title, value: Pretty Woman).
% The $j$-th metadata of the item $i$ is expressed in key-value form: $m_{i,j} = (k_{i, j}, v_{i, j})$, (\eg key: title, value: Pretty Woman).
The $j$-th metadata of item $i$ is represented in key-value form: $m_{i,j} = (k_{i,j}, v_{i,j})$, where $k_{i,j}$ is the key (\eg, \textit{title}) and $v_{i,j}$ is the corresponding value (\eg, \textit{Pretty Woman}).
% 이때 CRS는 t-1까지의 utterance를 기반으로 사용자가 추천해주기 적합한 아이템 $i_{t}$를 예측하는 것을 목적으로 한다.
In this case, the goal of the CRS is to predict the most suitable item $i_{t}$ to recommend to the user, based on the dialogue history consisting of utterances up to turn $t-1$.

\noindent \textbf{Retrieval-based CRS.}
% Retrieval-based CRS는 recommendation task를 retrieval 형태로 reformulate한다.
% 구체적으로, dialogue $c_u$의 $t-1$까지의 utterance를 text representation $T_u$로,  item $i$의 textual metadata $m_i$를 활용하여 $T_i$로 변환한다.
Retrieval-based CRS reformulates the recommendation task as a retrieval problem. Specifically, it transforms the utterances up to turn $t-1$ in the dialogue $c_u$ into a text representation $T_u$, which is then used to retrieve items by leveraging the textual metadata $m_i$ associated with item $i$.
Then, the score $S(u, i)$ between the user $u$ and item $i$ is calculated as follows:
\begin{equation}
    S(u, i) = \text{Ret}(T_u, T_i),
\end{equation}
where $\text{Ret}(\cdot)$ represents the retriever, which calculates the similarity between the user's text representation $T_u$ and the item's metadata $m_i$.

\subsection{Preference Extraction}
While existing methods rely on knowledge graphs or review data, we leverage LLMs to extract like/dislike preference information. The advantages of using LLMs for this purpose are as follows:
\textit{(i) Sentiment classification:} In dialogue,user express wide range of preference (\eg, prefer, abhor, thrills).
LLMs can effectively distinguish the sentiment of them by understanding the context and classify into ``like'', or ``dislike''.
\textit{(ii) Leverage LLM's reasoning skills to infer complex preferences:} LLMs provide advanced reasoning capabilities, enabling them to infer nuanced user preferences that go beyond explicit expressions in conversations.

% In particular, 우리는 dialog history를 기반으로 User preference를 extraction하고, item의 metadata와 review를 종합하여 user가 item에 갖는 general한 preference를 추출하며, 사용한 모델은 gpt-3.5-turbo이다. ~\cite{crs-dataset2024pearl}에서는 ChatGPT를 사용하여 리뷰로부터 사용자의 like/dislike persona를 효과적으로 추출하였으며, 우리도 효과적으로 사용자의 preference를 추출하기 위해 선행 연구의 프롬프트와 동일한 프롬프트를 사용하였고, task에 따라 조금씩 변경하였다.
% First, we extracted user preferences from the dialogue history to obtain each user preference.
% Next, to get the general user preferences for the item, we use item metadata and its reviews that have top-3 helpful votes. We utilized GPT-3.5-turbo as the underlying model for this process.
First, we extract individual user preferences from the dialogue history. Next, to infer general user preferences for an item, we utilize the item's metadata along with its top-3 most helpful reviews. ChatGPT serves as the underlying model for this process.
Following the approach in ~\cite{crs-dataset2024pearl}, where ChatGPT was successfully used to extract users' like/dislike personas from reviews, we adopt a similar prompt structure with slight modifications to better align with the specific requirements of our tasks.

\noindent \textbf{User Preference Extraction.}
% 우리는 사용자 선호를 추출하기 위해 dialogue를 기반으로 사용자가 좋아하는 특징과 싫어하는 특징을 추출하며 사용한 프롬프트는 다음과 같다.
To extract user preferences, we identify the features that users liked and disliked based on the dialogue. The prompts used for this extraction are as follows:

\vspace{-2mm}

\begin{tcolorbox}
\textbf{Prompt:}
\\
Given the conversation between the user and the system, describe what [User] likes and dislikes about movies as keyphrases, respectively. If there is nothing to mention about either like or dislike, simply write "None" under the corresponding tag.

Format example:
[Like] keyphrase 1, keyphrase 2, keyphrase 3...
[Dislike] keyphrase 1, keyphrase 2, keyphrase 3...

Here is a conversation between the user and the system: \{dialogHistory\}
\end{tcolorbox}

% 이러한 과정을 통해 user $u$는 list of like preference $L_u = (l_{u,1}, ..., l_{u, |L_u|})$를 얻게 된다, where $l_{u,j}$는 사용자 $u$가 선호하는 $j$번째 feature d(\eg Humorous entertainment) and $|L_u|$ denotes the 개수 of like feature of user $u$.
% 비슷한 방식으로, list of dislike preference $D_u = (d_{u,1}, ..., d_{u, |D_u|})$를 얻게 된다, where $d_{u,j}$는 사용자가 $u$가 선호하지 않는 $j$번째 feature (\eg Superhero movies) and $|D_u|$ denotes the 개수 of dislike features of user $u$.
% In this process, user $u$ gets a list of like preference $L_u = (l_{u,1}, ..., l_{u, |L_u|})$, where $l_{u,j}$ is the $j$th feature d (\eg, \textit{Humorous entertainment}) that user $u$ likes and $|L_u|$ denotes the number of like features of user $u$.
In this process, user $u$ receives a list of like preferences, denoted as $L_u = (l_{u,1}, ..., l_{u, |L_u|})$, where $l_{u,j}$ represents the $j$-th feature (\eg, \textit{Humorous entertainment}) that user $u$ likes, and $|L_u|$ indicates the total number of like features for user $u$.
% Similarly, we get a list of dislike preference $D_u = (d_{u,1}, ..., d_{u, |D_u|})$, where $d_{u,j}$ is the $j$th feature d (\eg, \textit{Superhero movies}) that user $u$ does not like and $|D_u|$ denotes the number of dislike features of user $u$.
Similarly, we obtain a list of dislike preferences, denoted as $D_u = (d_{u,1}, ..., d_{u, |D_u|})$, where $d_{u,j}$ represents the $j$-th feature (e.g., Superhero movies) that user $u$ dislikes and $|D_u|$ indicates the total number of dislike features for user $u$.

% Item preference를 추출해야 하는 이유
\noindent \textbf{Item Preference Extraction.}
% Item preference는 일반적으로 사람들이 해당 아이템에 대해서 좋아하거나, 싫어하는 특징들을 의미한다.
% To extract the preference features from the item, 우리는 IMDb website\footnote{https://www.imdb.com/}로부터 item의 metadata와 review를 crawled했다.
% 이러한 metadata와 review로부터 preference를 추출할 수 있는 가장 간단한 방식은 모두 concat하여 what user like and dislike about the item을 추론하는 것이다.
% To extract the preference features from the item, we crawled the item's metadata and reviews from the IMDb website\footnote{https://www.imdb.com/}.
% The simplest way to extract preference from these metadata and reviews is to concatenate them to infer what user likes and dislikes about the item.
To extract preference features from the item, we crawled the item's metadata and reviews from the IMDb website\footnote{https://www.imdb.com/}. The simplest method to extract preferences from this metadata and review data is to concatenate them, allowing us to infer what the user likes and dislikes about the item.
% 하지만 그렇게 할 경우, review에서 비슷한 내용을 다룰 경우 redundant한 preference가 생긴다.
However, if we simply express the preferences as plain text, this approach can lead to redundant information when the reviews and metadata cover similar content.
% 예를 들어, 3개의 review에서 "a", "b", "c"라는 말을 공통적으로 했을 경우, 비슷한 내용의 preference가 추출되게 된다. (예시로 보충 예정)
% 따라서 우리는 추출된 preference들을 기반으로 keyphrase를 추출하는 과정을 다시 한 번 거치며 data를 organize한다.
% 이렇게 함으로써 preference들을 취합하여 더 fundamental한 특징을 생성하여 데이터의 품질이 올라갈뿐만 아니라 전체 길이를 reduce할 수 있다.
Therefore, we refine the data by extracting keyphrases from the previously extracted preferences.
This process helps aggregate similar preferences into more fundamental features, enhancing data quality while also reducing the overall length and redundancy.
The example of item preference extraction is shown in figure ~\ref{fig:pref_extraction}.
In this example, after preference extraction, we can see that there are similar preferences (\eg, Top-notch playlist, Stella playlist). We can use keyphrase extraction to abbreviate these redundant preferences to something like ``Outstanding playlist''.
% 근거 부족함

% 구체적으로, 먼저 following 기존 연구~\cite{crs-dataset2024pearl}, metadata와 review로부터 사용자들이 어떤 점을 liked하고 disliked하는지 파악하기 위해 다음과 같은 prompt를 사용하여 사용자들이 focus하는 부분들 위주로 요약된 item feature를 획득하였다.
% Helpful vote 기준으로 가장 유용한 review 3개만 추출해서 사용하였다.
% 사용된 prompt의 예시는 다음과 같다.
In detail, we first extract item features that reflect what users focus on by referencing prior studies~\cite{crs-dataset2024pearl}, item metadata, and reviews to understand user likes and dislikes. We use the following prompts to summarize key user preferences, focusing only on the three most helpful reviews based on helpful votes. Below is an example of the prompts we used:
\begin{tcolorbox}
\textbf{Prompt:}
\\
You are a good user preference analyzer.
Given some popular reviews about {title}, describe what people liked and disliked about the movie, under [Like] and [Dislike] respectively. If there is nothing to mention about like/dislike, simply write "None." under the corresponding tag.
Here are some basic information about the movie and reviews about it:
Title: \{title\}
Genre: \{genre\}
Cast: \{cast\}
Director: \{director\}
Reviews: \{reviews\}
\end{tcolorbox}

% 위 prompt를 통해 추출된 preference를 다음 prompt를 사용하여 집약된 keyphrase로 변환한다.
The preferences extracted using the above prompt are then converted into aggregated keyphrases with the following prompt:
\begin{tcolorbox}
\textbf{Prompt:}
\\
You are a good user preference analyzer
Below are the common [Like] and [Dislike] from users about the movie {title}. Based on this information, generate 5-8 keyphrases that represent user preferences and intentions for this movie, separated by commas. Do not include any other explanations or sentences.

Here is some basic information about the movie and users' preferences information:

Preferences: \{preferences\}
\end{tcolorbox}

% 위 과정을 통해 item $i$는 list of like preference $L_i = (l_{i,1}, ..., l_{i,|L_i|})$를 얻게 된다, where $l_{i,j}$는 item $i$의 $j$번째 textual feature that 사람들이 일반적으로 선호하는 (\eg Funny scenes between main characters) and $|L_i|$ denotes the 개수 of like feature
% Through the above process, item $i$ gets a list of like preference $L_i = (l_{i,1}, ..., l_{i,|L_i|})$, where $l_{i,j}$ is the $j$th textual feature of item $i$ that users generally prefer (\eg, \textit{Funny scenes between main characters}) where $|L_i|$ denotes the number of like feature.
Through this process, item $i$ is assigned a list of like preferences, denoted as $L_i = (l_{i,1}, ..., l_{i,|L_i|})$, where $l_{i,j}$ represents the $j$-th textual feature of item $i$ that users generally prefer (\eg, \textit{Funny scenes between main characters}). $|L_i|$ indicates the number of like features.
% 그리고 list of dislike preference $D_i = (d_{i,1}, ..., d_{i,|D_i|})$를 얻게 된다, where $d_{i,j}$는 item $i$의 $j$번째 textual feature that 사람들이 일반적으로 dislike하는 (\eg Predictable scenes) and $|L_i|$ denotes the 개수 of dislike features of user $i$.
Similarly, we obtain a list of dislike preferences, denoted as $D_i = (d_{i,1}, ..., d_{i,|D_i|})$, where $d_{i,j}$ represents the $j$-th textual feature of item $i$ that people typically dislike (\eg, \textit{Predictable scenes}). $|D_i|$ indicates the number of dislike features.


\subsection{Preference-aware Representation}
In this section, we explain how \ours\ obtains a preference-aware representation that considers the user's multifaceted preferences. Specifically, it incorporates an additional preference-only representation to effectively model both the user and the item.
% While existing retriever-based LLM~\cite{crs-ret2023CRSRetbaseline} bm25를 retriever로 사용한 반면, 우리는 BERT을 backbone으로 갖는 dense retriever를 사용한다.
% vocabulary mismatch의 문제에서 벗어나 dense retirever의 뛰어난 문맥 이해를 기반으로 사용자 표현과 아이템 표현의 의미적 유사도를 파악할 수 있다는 장점이 있다.
% 따라서 우리는 Bi-encoder 구조의 dense retriever 차용하였으며, backbone model로 BERT~\cite{lm2019bert}를 사용하였다.

While existing retriever-based LLM methods, such as ~\cite{crs-ret2023CRSRetbaseline}, utilize BM25 as the retriever, we employ a dense retriever with BERT as its backbone. Dense retrievers offer the advantage of avoiding vocabulary mismatch, a common issue with sparse retrievers, and can effectively capture semantic similarities between user and item expressions due to their superior contextual understanding. Consequently, we implemented a dense retriever with a bi-encoder structure, using BERT~\cite{lm2019bert} as the underlying model.


\noindent
\textbf{User representation.}
% The textual representation of utterance at timestep $t$ of dialogue $c$ is $T_{c,1}$는 $r_t$와 $s_t$의 join이다(\eg [User] I am looking for a comedy movie.
% Dialogue $d$의 textual representation은 utterance의 textual representation을 concatenate함으로써 얻을 수 있다.
% \begin{equation}
% T_c = (T_{c,1}, T_{c,2}, ..., T_{c,t-1}) = ([r_1;s_1;...;r_{t-1}; s_{t-1}])
% \end{equation}
% 사용자의 like preference에 대한 textual representation $T_{u,l}$은
% 각 preference들을 concat하고 special token \texttt{[Like]}을 prepend함으로써 얻을 수 있다.
% dislike preference에 대한 textual representation $T_{u, d}$ 또한 같은 방법으로 concat한 후, special token\texttt{[Dislike]}을 prepend한다.
% 최종적으로 preference에 대한 textual representation $T_{u, p}$는 $T_l$과 $T_d$를 special token\texttt{[SEP]}으로 join함으로써 얻어질 수 있다.
The textual representation of the utterance at the $t$-th turn of dialogue $c$, denoted as $T_{c,t}$, is defined as the concatenation of $r_t$ and $s_t$ (e.g., [User] ``I am looking for a comedy movie''). The textual representation of the entire dialogue $d$ is then obtained by concatenating the textual representations of all its individual utterances as follows:

\begin{equation}
T_c = (T_{c,1}, T_{c,2}, ..., T_{c,t-1}) = ([r_1;s_1;...;r_{t-1}; s_{t-1}]).
\end{equation}
% The textual representation of the user's like preference, denoted as $T_{u,l}$ is obtained by listing each preference and prepending with the special token \texttt{[Like]}.
% The textual representation of the user's dislike preference, denoted as $T_{u, d}$, is similarly constructed by concatenating the individual preferences and prepending the special token \texttt{[Dislike]}.
% The textual representation $T_{u, p}$ of a user's preference can be obtained by joining $T_l$ and $T_d$ with the special token \texttt{[SEP]}:
The textual representation of the user's like preferences, denoted as $T_{u,l}$, is obtained by listing each preference and prepending the special token \texttt{[Like]}.
Similarly, the textual representation of the user's dislike preferences, $T_{u,d}$, is constructed by concatenating the preferences with the token \texttt{[Dislike]}. The user's overall preference representation, $T_{u,p}$, is then created by joining $T_{u,l}$ and $T_{u,d}$ with the token \texttt{[SEP]}:

\begin{align}
    & T_{u, l} = ([\texttt{[LIKE]};l_{u,1};...;l_{u,|L_u|}]) \\
    & T_{u, d} = ([\texttt{[DISLIKE]};d_{u,1};...;d_{u,|D_u|}]) \\
    & T_{u, p} = ([T_{u,l};\texttt{[SEP]};T_{u,d}]).
\end{align}

% 사용자의 textual representation $T_u$는 \texttt{[CLS]}와 dialogue text representation $T_c$, preference text representation $T_{u, p}$을 concat함으로써 얻어질 수 있다.
% List of contextualized된 word representation list $O_u$를 얻기 위해서 우리는 $T_u$를 tokenize한 후 PLM에 통과시킨다, where d is the hidden dimension size of the PLM and $o \in \mathbb{R}^d$

The textual representation of user $u$, denoted as $T_u$, is formed by concatenating the \texttt{[CLS]} token, the dialogue text representation $T_c$, and the preference text representation $T_{u,p}$. To obtain the list of contextualized word representations, denoted as $O_u$, we tokenize $T_u$ and pass it through the BERT model as follows:

\begin{equation}
\begin{aligned}
    [x_\texttt{[CLS]}, x_1,...,x_{L_u}] & = \text{Tokenize}(T_u) \\
    & = \text{Tokenize}([\texttt{[CLS]};T_c;T_{u,p}] \\
    O_u = [o_{\texttt{[CLS]}}, o_1,...,o_{L_u}]  & = PLM([x_\texttt{[CLS]}, x_1,...,x_{L_u}]).
    \end{aligned}
\end{equation}

% where $x \in \mathcal{V}$는 tokenized token, $L_u$은 tokenize 이후의 $(T_u)$의 길이, $o_l$는 last hidden state of $x_l$ after passing pre-trained language model.

% 여기서 우리는 사용자 표현과 사용자 선호 표현을 얻는다.
% 먼저 사용자 표현 $h_u$로는 \texttt{[CLS]} token의 contextualized representation인 $o_{\texttt{[CLS]}}$를 사용하며, 사용자 선호 표현  ${h_u}^{pref}$으로는 $x_l\in T_{u,p}$인 $o_l$들의 average 값을 사용한다.
% It can be 
Let $x \in \mathcal{V}$ represent a tokenized token, $L_u$ denote the length of $T_u$ after tokenization, and $o_l$ be the last hidden state of $x_l$ after passing through the pre-trained language model.

From this, we derive both the user representation and the user preference representation. Specifically, we use $o_{\texttt{[CLS]}}$, the contextualized representation of the \texttt{[CLS]} token, as the user representation $h_u$. Additionally, the user preference representation, ${h_u}^{pref}$, is obtained by taking the average value of $o_l$ for $x_l \in T_{u,p}$:

\begin{align}
    h_u &= o_{\texttt{[CLS]}}, \text{where} \, o_{\texttt{[CLS]}} \in O_u\\
    {h_u}^{\text{pref}} &= \text{Mean}(o_l \mid o_l \in O_u, x_l \in T_p).
\end{align}

\noindent
% \textbf{Item representation.} Item representation 역시 비슷한 방식으로 진행된다.
% Item $i$의 metadata $M_i$ can be represented in text as $T_m = ([k_{i, j}, v_{i, j},...,k_{i,{|M|}}, v]_{i,{|M|}})$
% Item preference에 대한 textual representation $T_{i,l}$과 $T_{i,d}$는 user와 동일한 방식으로 각 like, dislike에 해당하는 preference들을 concat하고. special Token \texttt{[Like]}, \texttt{[Dislike]}를 prepend함을써 얻을 수 있다.
% $T_{i,p}$ 또한 동일하게 $T_{i,l}$, \texttt{[SEP]}와 $T_{i,d}$를 연결해서 얻는다.
% 아이템의 textual representation $T_i$는 \texttt{[CLS]}와 metadata text representation $T_m$, preference text representation $T_p$을 concat함으로써 얻어질 수 있다.
% tokenized된 최종 표현은 다음과 같다.
\textbf{Item representation.} he item representation is constructed in a similar manner to the user representation. The metadata of item $i$, denoted as $M_i$, is represented in text form as: $T_m = ([k_{i, j}, v_{i, j},...,\\k_{i,{|M|}}, v]_{i,{|M|}})$.
The textual representations $T_{i,l}$ and $T_{i,d}$, which correspond to the item's like and dislike preferences, are constructed by concatenating the respective preferences, prepending them with the special tokens \texttt{[Like]} and \texttt{[Dislike]} in the same way as for the user. The combined preference representation, $T_{i,p}$, is then created by concatenating $T_{i,l}$, \texttt{[SEP]}, and $T_{i,d}$.
The final textual representation $T_i$ of item $i$ is formed by concatenating \texttt{[CLS]}, the metadata text representation $T_m$, and the preference text representation $T_{i,p}$. The tokenized representation is then:

\begin{equation}
\begin{aligned}
    [x_\texttt{[CLS]}, x_1,...,x_{L_i}] & = \text{Tokenize}(T_i) \\
    & = \text{Tokenize}([\texttt{[CLS]};T_m;T_{i,p}] \\
    O_i = [o_{\texttt{[CLS]}}, o_1,...,o_{L_i}]  & = PLM([x_\texttt{[CLS]}, x_1,...,x_{L_i}])
\end{aligned}
\end{equation}

% 이 사용자와 동일하게 tokenized된 표현을 PLM에 집어넣고, 표현을 pool하는 과정을 거쳐 $h_i$와 ${h_i}^{pref}$를 얻게 된다.
% We put the same tokenized representation as this user into PLM, pool the representations, and get $h_i$ and ${h_i}^{pref}$ as follow:
We feed this tokenized item representation into the pre-trained language model (PLM) in the same way as the user representation. By pooling the representations, we obtain the item representation $h_i$ and the item preference representation ${h_i}^{pref}$ as follows:
\begin{align}
    h_i &= o_{\texttt{[CLS]}}, \text{where} \, o_{\texttt{[CLS]}} \in O_i \\
    {h_i}^{\text{pref}} &= \text{Mean}(o_l \mid \in O_i, x_l \in T_{i,p}).
\end{align}


\noindent
\textbf{Prediction.}
% 위에서 구한 사용자와 아이템 점수를 기반으로 둘의 점수를 계산한다.
% 이건 preference를 고려하는 간단하고 직관적인 방법이다.
% similarity function은 dot product를 쓴다.
% Calculate their scores based on the user and item scores obtained above. This is a simple and intuitive way to take preference into account. For the similarity function, use dot product as follows:
To calculate the scores based on the user and item representations obtained above, we compute their similarity using the dot product, which is straightforward and effectively incorporates user preferences into the scoring process. The score $S(u, i)$ between user $u$ and item $i$ is computed as follows:
\begin{equation}
    S(u, i)  = {h_u}^\top h_i + {{h_u}^{pref}}^\top {h_i}^{pref}.
\end{equation}

\subsection{Preference-aware Alignment Training}
% 우리는 둘 사이의 gap을 bridge하는 것을 에임으로 한다.
% 기존 연구는 이걸 못하고 있다 retriever를 학습 안해서
% 그래서 우리는 ~를 ~ 하는 preference-aware alignment training을 제안한다.
% 이것은 두 가지 task: (i) user-item contrastive learning과 (ii) Preference-level contrastive learning으로 구성되어 있다.
% user-item contrastive learning은 기존 dpr과 동일한 방식으로 학습한다.
% preference-level contrastive learning은 user와 item의 preference를 align하는 부분으로, 이로 하여금 retriever가 semantic similarity뿐만 아니라 preference similarity까지 고려할 수 있도록 한다.

% in-batch negative를 쓴다

We aim to bridge the gap between language models and user preferences by proposing a \textit{preference-aware alignment training approach}, which aligns models with multifaceted user preferences. This consists of two key tasks: (i) user-item contrastive learning and (ii) preference-level contrastive learning.
The user-item contrastive learning is trained in the same way as traditional DPR. The preference-level contrastive learning is the part that aligns the preference of user and item, which allows the retriever to consider not only semantic similarity but also preference similarity.
User-item loss $\mathcal{L}_{\text{seq}}$ and preference-alignment loss $\mathcal{L}_{\text{pref}}$ can be formulated as:

\begin{align}
    \mathcal{L}_{\text{seq}} & = - \log\frac{\exp\left( h_u^\top {h_i^+} / \tau \right)}{\sum_{i \in \mathcal{B}} \exp\left( h_u^\top {h_i^-} / \tau \right)} \\
    \mathcal{L}_{\text{pref}} & = - \log\frac{\exp\left( {h_u^{\text{pref}}}^\top {h_i^{\text{pref}}}^+ / \tau \right)}{\sum_{i \in \mathcal{B}} \exp\left( {h_u^{\text{pref}}}^\top {h_i^{\text{pref}}}^- / \tau \right)},
\end{align}
where $\tau$ is a hyperparameter, and adopt in-batch negative for training.

% 따라서 \ours를 학습하기 위해 우리는 multi-task strategy를 적용하며, 최종 loss는 다음과 같다.
Therefore, to train \ours, we adopt a multi-task learning strategy. The final loss is a combination of both the user-item contrastive loss and the preference-level contrastive loss, formulated as follows:
\begin{equation}
    \mathcal{L} = \mathcal{L}_{seq} + \gamma \cdot \mathcal{L}_{pref},
\end{equation}
where $\gamma$ is a hyperparameter that controls the ratio of the two losses.


% 전개 고민: user preference에 대한 전반적인 조사로 갈지, 아예 제안 방법으로 갈지

% In this section, 우리는 CRS에서 효과적으로 사용자의 preference를 고려한 item search를 가능하게 하는 프레임워크인 \textcolor{red}{Ours}를 제안한다. First, (i) LLM을 통해 입력된 대화로부터 사용자의 like와 dislike 선호를 추출한다. (i) Retrieval는 입력된 사용자의 대화. 우리는 가장 간단한 프레임워크를 사용해보았다.

% \subsection{Problem Definition}

% \subsection{Dataset}
% \subsection{Data Construction}\label{sec:dataset}
% % 학습을 위한 dataset 구축
% In this section, 우리는 preference-aware retrieval 학습을 위해 사용자 발화 및 상품에 대한 user preference dataset을 구축한다. gpt-3.5-turbo-0125를 이용하여 데이터셋을 구축하였고, 사용한 프롬프트는 ~\cite{dataset2024pearl}에서 영감을 받아 동일한 프롬프트를 domain에 맞게 변경하여 사용하였다.
% 데이터셋을 어떻게 생성했느냐면, document에서는 2-stage로 구분이 된다. 첫 번째 스테이지에서는 먼저 모든 아이템에 대한 리뷰를 수집한다. 그리고 helpful vote가 많은 순으로 5개를 선택하고 얘네들을 프롬프트에 넣어서 [Like]랑 [Dislike]를 구분해서 뽑아달라고 부탁한다. 그러면 plain text 형태로 그러한 결과들이 주르륵 나오게 되는데, 그렇다면 두 번째 단계로 keyphrase를 추출해달라고 한다. 우리는 BERT를 쓸 것이고  token length 제한이 있기 때문에 이럴 수밖에 없었다! 그러면 이제 또 keyphrase를 추출해준다.
% 그렇다면 대화에서는 어떻게 하냐면, 그냥 대화만 제공하고 여기서 like, dislike를 keyphrase 형태로 바로 뽑아달라고 한다. 그러면 뽑아준다. 뽑힌 예시는 Figure X와 같다. 데이터셋별로 뽑힌 keyphrase의 양상이 다른데, 이것은 나중에 설명하든가 아니면 지금 설명하든가 아니면 빼든가 해야겠다!

% (revcore 문구, 페러프레이징 필요) To construct a review database, we crawled 30 reviews for each movie from IMDb website, which is one of the most popular and authoritative movie databases.
% In pratice, we select the 30 reviews with the highest helpful scores for each movie to guarantee the high quality of collected reviews.

% \subsection{Prosed Model}

% special token을 더하고 \ours이를 BERT를 통과시킨다. 
% \[
% \mathbf{E}_X = \left[\mathbf{E}_{[\text{CLS}]}, \mathbf{E}_{w_1}, \mathbf{E}_{[\text{LIKE}]}, \mathbf{E}_{[\text{SEP}]}, \dots, \mathbf{E}_{w_l}, \mathbf{E}_{[\text{SEP}]}\right]
% \]
% 그리고 user sequence에 대해서는 전체에 대해, Like에 대해서는 Like 토큰부터 Sep까지 mean pooling을 하여 더한다.


% \[
% \mathcal{L}_\textit{{\text{user}}} = -\log \frac{\exp \left(\text{sim}\left(\mathbf{u}_\textit{{\text{seq}}}, \mathbf{I}_i^{+}\right) / \tau \right)}{\sum_{i \in \mathcal{I}} \exp \left(\text{sim}\left(\mathbf{u}_\textit{{\text{seq}}}, \mathbf{I}_i\right) / \tau \right)}
% \]

% \[
% \mathcal{L}_\textit{{\text{pref}}} = -\log \frac{\exp \left(\text{sim}\left(\mathbf{u}_\textit{{\text{pref}}}, \mathbf{I}_i^{+}\right) / \tau \right)}{\sum_{i \in \mathcal{I}} \exp \left(\text{sim}\left(\mathbf{u}_\textit{{\text{pref}}}, \mathbf{I}_i\right) / \tau \right)}
% \]

% \[
% \mathcal{L} = \mathcal{L}_\textit{{\text{user}}} + \alpha \cdot \mathcal{L}_\textit{{\text{pref}}}
% \]



==> body/WSDM/4_experiment.tex <==


\input{tables/tab_main}

\section{Experimental Setup}\label{sec:experimental_setup}
\textbf{Datasets.}
To evaluate the performance of \ours, we conduct experiments on the Pearl~\cite{crs-dataset2024pearl} dataset in the movie domain, as well as the MobileConvRec ~\cite{crs-dataset2024mobileconvrec} dataset from the Google Play Store.
As pointed out in previous studies~\cite{crs-llm2023llmzs}, using items mentioned in the conversation as ground truth can be unnatural in recommendation environments. It may lead to issues such as memorization in learning-based models.
Therefore, we remove repeated items mentioned in the dialogue in this paper.
Additionally, ground-truth instances for which no metadata was available were excluded from the analysis.
Table~\ref{tab:statistics} presents the dataset statistics after the aforementioned preprocessing.

\noindent \textbf{Baselines.} To assess the effectiveness of \ours, we divide the evaluation into three groups: learning-based methods, LLM zero-shot methods, and retrieval-augmented methods. This categorization allowed us to comprehensively evaluate the effectiveness of the proposed approach.

\setlength{\parindent}{1em}(i) Learning-based:
\begin{itemize}[leftmargin=10mm]
\item \textbf{UniCRS~\cite{crs2022unicrs}}: It employs a unified architecture that combines conversational and recommendation tasks, leveraging a pre-trained model fine-tuned on large conversational datasets to generate context-aware recommendations.
\end{itemize}

\setlength{\parindent}{1em}(ii) LLM zero-shot:
\begin{itemize}[leftmargin=10mm]
\item \textbf{LLM}~\cite{crs-llm2023llmzs}: We evaluate the zero-shot performance of ChatGPT\footnote{https://openai.com/} (gpt-3.5-turbo-0125) generating item title given user dialogue without any task-specific fine-tuning.
\end{itemize}

\setlength{\parindent}{1em}(iii) Retrieval-based:
\begin{itemize}[leftmargin=10mm]
\item \textbf{BM25~\cite{RobertsonW94BM25}}: BM25 is used as a traditional retrieval model that ranks items based on their term relevance to the dialogue context, retrieving the most relevant items from a pre-existing index.
\item \textbf{Dense search~\cite{ir2020dpr}}: Dense search without fine-tuning, uses dense vector representations to match the dialogue context with items, retrieving items based on the similarity between their pre-trained embeddings and the encoded dialogue.
\end{itemize}
% 또한, 우리는 LLM zero-shot 및 retrieval baseline에 대해 preference 있고 없고 variant를 추가해서 실험하였다.
% LLM zero-shot (w/)의 경우 dialogue에 user preference를 \ours와 동일하게 concat해주었으며, retrieval basedline의 경우 dialogue와 item 모두에 preference를 추가하였다.
Additionally, we conduct experiments by introducing variants with and without user preferences for both the LLM zero-shot and retrieval baseline methods.
In the case of LLM zero-shot (w/), user preferences were concatenated to the dialogue, similar to \ours. For the retrieval baseline, preferences were added to both the dialogue and item representations.

\noindent \textbf{Evaluation Settings.}
To evaluate the recommendation performance within the CRS, we utilize the widely used metrics NDCG@k and Recall@k (with k=1, 10, 50) in the recommendation domain. 
% NDCG@k measures the ranking quality of the recommended items by considering the position of the correct items in the ranked list.
% Recall@k calculates the proportion of relevant items successfully retrieved within the top-k recommendations.
Following previous research~\cite{crs-llm2023llmzs}, we exclude repeated items from the ground-truth set to ensure a more accurate assessment. 

\noindent \textbf{Implementation Details.}
We implement \ours\,based on Huggingface's BERT model\footnote{https://huggingface.co/transformers/}.
The training process is conducted using the bf16 precision format to enhance computational efficiency and reduce memory usage without sacrificing model performance.
Note that when extracting user preferences from dialogues in the Pearl dataset, we did not employ the two-stage extraction method.
Instead, keyphrases were directly extracted from the user persona provided for each dialogue in the Pearl dataset.
% a search는 [0.25, 0.5, 1, 1.25, 1.5]에서 했고, Pearl과 MobileConvRec은 0.5, Redial은 1을 사용하였다. learning rate으로는 5e-5로 설정하였고 Adam optimizer를 사용하였으며, REcall@10으로 earlpy stop with patience 5하였다. For the baseline, UniCRS는 저자의 코드를 사용하였으며, MobileConvRec은 knowledge graph가 side information에 없기 때문에 돌리지 못하였다. Pearl의 성능은 제안된 논문에서 가지고 왔다. For the BM25, we utilize the Pyserini library~\cite{bm252021pyserini} to perform the retrieval tasks. dense search는 sentence-transformer를 사용하여 구현하였다.
The hyperparameter search for the $\gamma$ parameter is conducted within the range of [0.25, 0.5, 1, 1.25, 1.5], with the optimal values set to 1.5 for Pearl and 0.5 for MobileConvRec. The learning rate is configured as 5e-5, using the Adam optimizer. $\tau$ is set as 1 for Pearl and 2 for MobileConvRec.
For model evaluation, we employed Recall@10 as the stopping criterion with early stopping set at 5 epochs of patience.
Since UniCRS requires a knowledge graph, which is not present in our two datasets, the performance of Pearl was sourced from the original paper~\cite{crs-dataset2024pearl} proposing the method, and MobileConvRec could not be evaluated.
For BM25-based retrieval tasks, we employed the Pyserini library~\cite{bm252021pyserini}, while the dense search is implemented using the sentence-transformer framework.

==> body/WSDM/5_results.tex <==
\input{Tables/tab-popularity}
\input{Tables/tab-coverage}

\section{Results and Analysis}\label{sec:results}
\subsection{Overall Performance}\label{sec:overall_performance}
We compared the performance of \ours\,against the baseline using two datasets across two distinct movie and application domains.
The experimental results are presented in Table~\ref{tab:main_table}.
% 학습 기반 메서드와 비교했을 때, \ours는 UniCRS와 비슷한 성능을 보였다. \ours는 UniCRS보다 구조가 비교적 간단하지만, 효과적으로 성능을 발휘할 수 있음을 확인할 수 있다. LLM zero-shot과 비교했을 때, Pearl과 MobileConvRec에서 기존의 LLM zero-shot 성능을 능가하는 결과를 보였다. 이는 retriever를 학습시킴으로써 사용자의 선호도를 더욱 잘 반영할 수 있었음을 의미한다.
% 특히, Retrieval-augmented 메서드와의 비교에서 BM25와 DPR를 비교했을 때, 의미적 유사성을 고려하는 것이 더 우수한 성능을 나타냄을 확인하였으며, 특히 BM25에 사용자 선호도 정보를 추가했을 때 더 높은 성능을 나타냈다.
% 여기서 주목할 정은 MobileConvRec에서 \ours의 성능이다.
% 기존 LLM 위주 방법론들은 LLM 내부의 world-knowledge에 크게 의존했기 때문에 LLM이 익숙한 도메인 (\eg Movie)에서만 실험을 진행할 수 있었다.
% 하지만 \ours는 LLM의 내부 지식을 사용자와 아이템 표현을 enhance할 수 있는 tool로서 활용하기 때문에 LLM의 limitation에 구애 받지 않으며 이를 활용하여 높은 성능을 보일 수 있다.
Overall, \ours outperforms baseline on all datasets
Compared to the learning-based method, \ours outperformed UniCRS, despite its relatively simpler structure, highlighting its effectiveness.
The comparison with LLM zero-shot methods indicates that training the retriever allowed for a better reflection of user preferences.
Notably, in comparisons with Retrieval-augmented methods, we found that untrained retriever struggles to identify user preferences.
Furthermore, when comparing w/o and w variants, we can see that there are cases where the extracted preference information is not helpful.
This highlights the importance of alignment, as simply adding preference information can actually degrade performance due to misalignment between semantic similarity and preference.

A key point of interest is \ours's performance on the Mobile. dataset.
Unlike traditional LLM-based methods, which heavily rely on the internal world knowledge of LLMs and are typically tested only in familiar domains (e.g., movies), \ours, leverages LLMs as tools to enhance user and item representations.
This allows \ours, to operate effectively without being constrained by the limitations of LLMs, resulting in superior performance across various domains.

\subsection{Popularity Bias} \label{sec:popularity_bias}
In this section, we empirically demonstrate the robustness of \ours\, against popularity bias in comparison to LLMs.
In this context, ``Head'' denotes the top 20\% of popular items among all ground-truth items, while ``Tail'' refers to the remaining 80\% items.
The result in Table ~\ref{tab:popularity} reveals that \ours\, exhibits robustness to popularity bias compared to LLMs, offering more satisfactory recommendations for the Tail group in both the Pearl and MobileConvRec datasets.
These results suggest that LLMs are vulnerable to popularity bias and \ours\, demonstrates stable performance with a marginal gap between the Head and Tail groups.

\subsection{Coverage} \label{sec:coverage}
% Table ~\ref{tab:coverage}은 세 가지 데이터셋에 대해 LLM zero-shot과 \ours에서의 coverage 나타낸다. 
% coverage는 전체 아이템 셋 $I$에 대해 모델이 생성한 결과가 얼만큼 전체 아이템 셋을 얼만큼 커버하는지 나타내는 지표로 $Rec/|I|$로 계산된다. 
% 실험 결과, LLM이 생성한 결과는 전체 아이템셋 중 Pearl에서는 약22\%, REDIAL에서는 약 35\%를 커버하며, APP에서는 커버하는 아이템 수가 약 11\%에 불과하다는 것을 확인할 수 있다. 
% 또한, LLM이 생성한 아이템 중 out-of-dataset item(OOD)의 경우, APP의 경우 무려 88\%에 육박하며, LLM과 \ours의 성능 차이가 왜 이렇게나 큰지를 보여준다. 
% 이는 LLM이 APP에 대한 internal knowledge가 비교적 부족하다는 것을 말해준다. 
% 반면, \ours의 경우, retriever 내의 아이템을 추천하는 것이기 때문에 OOD는 존재하지 않는다. 또한, coverage는 LLM보다 높으며 비교적 다양한 아이템을 추천하여 제공한다는 것을 알 수 있다.
Table ~\ref{tab:coverage} presents the coverage comparison between LLM zero-shot and \ours\, across two datasets.
Coverage is defined as the proportion of the total item set $I$ that is covered by the model's generated results at cutoff 20.
The items generated by LLM cover approximately 22\% of the total item set in the Pearl dataset, on the other hand, in the MobileConvRec dataset, 88\% of the items generated by LLM were out-of-dataset (OOD), illustrating the significant performance gap between LLM and \ours.
This suggests that LLM has relatively limited internal knowledge of the APP domain.
In contrast, \ours\, does not produce any OOD items since it exclusively recommends items from the retriever's item set.
Additionally, \ours\, exhibits higher coverage than LLM, indicating that it recommends a broader and more diverse range of items.
This highlights the superior performance of \ours\, in generating relevant and diverse recommendations compared to LLM, especially in domains where LLM's internal knowledge is limited.

\input{Tables/tab-ablation}
\input{Figures_tex/fig_case_study}

\subsection{Ablation Study}
In Table ~\ref{tab:ablation}, we analyze how our component, preferences, preference-aware representation, and preference-aware alignment training affect performance in two datasets.
In this experiment, we sampled half of the training data of Pearl for efficiency.
In variant (1), we do not use the preference representations ${h_u}^{\text{pref}}$ and ${h_i}^{\text{pref}}$, and we do not utilize the preference-alignment loss $\mathcal{L}_{\text{pref}}$.
Variants (2) and (3) eliminate user preferences $P_u$ or item preferences $P_i$, respectively.
Since there is no user-item preference-aware representation pair, we only use $L_{seq}$ to train these variants.
Lastly, variant (4) removes preferences, preference-aware representation, and preference-aware alignment, which is the simplest form of training dense retriever.
First, we can validate the effectiveness of preference-aware representation and preference-aware alignment training.
The sub-optimal performance of variant (1) compared to Ours shows that the gap between preference and semantic similarity cannot be fully exploited by adding preference alone and that \ours effectively bridges this gap.
We also investigate the effect of $P_u$ and $P_i$ by comparing variants (1), (2), (3), and (4).
We can see that variants (1), (2), and (3) perform better than variants (4), which do not use any preference, and that $P_i$ is vital compared to $P_u$.
We speculate that this is because $P_u$ is information implicitly included in the dialog, while $P_i$ is information newly extracted through review.
However, in MobileConvRec, there is no significant difference in performance with or without preference.
This is due to the nature of MobileConvRec's data: the dialogue focuses on the aspects of the app itself (Apps with at least 10M reviews, Average rating of 4.7 stars or higher), while the reviews of the actual app are based on the user experience in the app(\eg, Great app for writing music over PDFs, Beautiful new graphics).


\subsection{Case Study}
% Figure 4는 Pearl 데이터셋에서 \ours가 정답으로 맞춘 경우에서 가장 like와 dislike가 바람직한 형태로 잘 모델링 된 것을 나타낸다.. 가장 바람직한 형태는 user preference 중 like 정보와 item like 정보가 유사한 것과, user preference의 dislike와 item의 like가 서로 반대되는 개념이어야 하고, item dislike와 비슷해서는 안되는 상태가 가장 바람직한 경우이다. 같은 색으로 하이라이팅 되어 있는 것은 같은 개념을 갖는 keyphrases를 의미한다. Figure 4에서 보이는 것처럼 사용자의 'Like'에 있는 구체적인 선호 Well-done lead characters가 맞춘 ground-truth의 Masterful character building, Deeply complex characters에 대응하며, 'Dislike'의 Disappointing portrayal of female characters와 반대되는 개념임을 확인할 수 있다. 또한, Dislike에 있는 Lana Turner's unconvincing acting, Stilted dialogue and histrioning acting은 Item에 대한 common like preferences인 Great acting과 반대되는 개념이다. 즉, Figure 1에서 나타난바와 같이 단순히 lexical matching이나 사용자의 like/dislike preferences를 전혀 고려하지 않고 item search를 하는 것이 아니라, user preference aware search를 한다는 점에서 제안한 preference-aware alignment training의 효과성을 정성적으로 확인할 수 있다.
Figure ~\ref{fig:case_study} illustrates a case in the Pearl dataset where \ours\, successfully models the relationship between the user's preferences and the item's characteristics, capturing both 'like' and 'dislike' information in a well-structured manner.
The most ideal scenario is when the user's 'like' preferences align closely with the item's positive attributes, while the user's 'dislike' preferences are opposed to those same positive aspects. Furthermore, the user's 'dislike' should not resemble the item's negative characteristics. The keyphrases highlighted in the same color represent concepts that share similar meanings.

As shown in Figure ~\ref{fig:case_study}, the specific preference in the user's ``Like'' section, ``Well-done lead characters'' colored with green aligns well with the ground-truth item's attributes such as ``Masterful character building'' and ''Deeply complex characters''.
Moreover, there is a clear opposition between the preference in the user's ``Dislike'' section, ``Disappointing portrayal of female characters, Lack of realism in Rhoda's behavior'', thereby further validating the model's preference alignment.
Additionally, preferences listed under ``Dislike'' such as ``Lana Turner's unconvincing acting'' and ``Stilted dialogue'' are opposite of “Great acting” and “Beautifully written dialogue,” which have the same color as themselves, orange and purple, respectively.
This alignment confirms that, unlike a simple lexical matching approach or an item search that ignores the user's like/dislike preferences, \ours\, performs a recommendation addressing user preferences.
This demonstrates the effectiveness of the proposed preference-aware alignment training, as it qualitatively captures the nuanced relationship between user preferences and item characteristics.

==> body/WSDM/6_conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
% 본 연구에서는 발화로부터 사용자의 like/dislike preferences 정보를 추출하고 이를 명시적으로 학습에 반영하여 retriever가 multifaceted preferences를 고려한 아이템 검색이 가능하도록 하는 novel framework인 \ours를 제안한다. 특히, retriever 학습 단계에서 preference-aware를 고려한 alignment training 방법을 통해 단순한 text similarity matching이 아니라 사용자의 like/dislike preference를 고려한 검색이 가능하도록 하여 사용자와 가장 관련된 상품을 찾을 수 있도록 했다. Pearl과 APP 데이터셋에서 제안 방법은 다른 learning-based, LLM zero-shot 방법을 outperform하였고, ReDial 데이터셋에서는 낮은 성능을 보이지만, Tail 그룹에 대해 Recall@1에서 약 63.51\%의 개선을 보이며 popularity bias에 강건한 모습을 보인다(Section 5.2). 또한, LLM zero-shot과 비교하여 높은 coverage를 보이며 아이템 셋 내에서 다양한 아이템을 커버하는 것을 확인할 수 있다(Section 5.3). 
In this study, we propose a novel framework, \ours, which extracts users' like/dislike preferences from their utterances and explicitly incorporates this information into the training process, enabling the retriever to consider multifaceted preferences when searching for items.
Specifically, during the retriever training phase, the preference-aware alignment training method allows  \ours\, to go beyond simple text similarity matching and perform searches that reflect users' like/dislike preferences, allowing it to find the most appropriate items for the user. 
On the Pearl and MobileConvRec datasets, the proposed method outperforms other learning-based and LLM zero-shot methods. 
Furthermore, compared to LLM zero-shot, the proposed method exhibits robustness against popularity bias and higher coverage, confirming its ability to cover a wider range of items within the item set.

==> body/WSDM/misc.tex <==
%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
\begin{CCSXML}
<ccs2012>
 <concept>
  <concept_id>00000000.0000000.0000000</concept_id>
  <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
  <concept_significance>500</concept_significance>
 </concept>
 <concept>
  <concept_id>00000000.00000000.00000000</concept_id>
  <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
  <concept_significance>300</concept_significance>
 </concept>
 <concept>
  <concept_id>00000000.00000000.00000000</concept_id>
  <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
  <concept_significance>100</concept_significance>
 </concept>
 <concept>
  <concept_id>00000000.00000000.00000000</concept_id>
  <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
  <concept_significance>100</concept_significance>
 </concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Do Not Use This Code~Generate the Correct Terms for Your Paper}
\ccsdesc[300]{Do Not Use This Code~Generate the Correct Terms for Your Paper}
\ccsdesc{Do Not Use This Code~Generate the Correct Terms for Your Paper}
\ccsdesc[100]{Do Not Use This Code~Generate the Correct Terms for Your Paper}

%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
\keywords{Do, Not, Us, This, Code, Put, the, Correct, Terms, for,
  Your, Paper}
  
\received{20 February 2007}
\received[revised]{12 March 2009}
\received[accepted]{5 June 2009}


==> body/backup/1_introduction_backup.tex <==
\input{figures/figures_tex/fig_motivating}
\section{Introduction}
\label{sec:introduction}

% 1. CRS 설명, 두 가지 Task 설명
% 2. 기존 CRS 소개 및 한계점
%  - 1) KG vs. LLM vs. Retrieval-based CRS
%  - 2) emotion-aware vs. non-emotion-aware
% 3. Retriever CRS (위 두 방법 대비 어떤 장점이 있는지)
% 4. Challenges (하지만 무엇을 해결하지 못했는지)
% 5. Contribution


% \textcolor{red}{
% 1. CRS 설명 (Task 설명, 어려운 이유) \\
% 2. 기존 연구 설명 (KG based, LLM based, 각각의 특징과 한계) \\
% 3. Retriever CRS (위 두 방법 대비 어떤 장점이 있는지) \\
% 4. Challenges (하지만 무엇을 해결하지 못했는지) \\
% 5. Contribution \\
% }

% Feedback
% 1. CRS 설명
% 2. 기존 연구
%     - KG based: Entity간 복잡한 관계를 잘 모델링하긴 하지만, KG에 의존적
%     - LLM-based: world knowledge와 reasoning ability가 있으나, 새로운 지식을 반영하기 어려움
%     - IR-based: 새로운 아이템 추천하기는 하지만 사용자의 preference는 서로 상반될 수 있기 때문에(like, dislike) 서로 다른 의도로 취급하여 검색을 해야 함
% 3. 기존 연구의 challenge
%     - 1. Conversation에 숨겨진 like/dislike를 어떻게 잘 찾을 수 있을까?
%         - 기존 IR은 단일하고 명시적인 query 의도를 갖기 때문에 이를 CRS에 그대로 활용하는 것은 적절치 않다.
%     - 2. 사용자의 Like/dislike를 어떻게 잘 고려해서 검색 추천을 할 수 있을까?
% 4. 제안 방법
% }

% 1. CRS 설명, 두 가지 task 설명, 기존 방식의 한계 간략하게 언급
In recent years, Large Language Models (LLMs) have accelerated the advancement of Conversational AI, leading to a growing interest and demand for Conversational Recommender Systems (CRS).
CRS yields personalized recommendations by deeply understanding the user's context and needs through real-time interactions. 
% It enhances the user's personalized experience by providing recommendations that are more aligned with their personalized preferences and evolving requirements.
CRS가 수행하는 task는 크게 두 가지로 구분된다: 텍스트로부터 사용자의 의도를 이해하고 적절한 추천을 제공하는 recommendation task와 사용자에게 적절한 응답을 제공하는 generation task.
In this paper, 최근 LLM의 발전이 자연어 생성에 있어서 naturalness를 향상시켰기에, we focus on the recommendation rather than the generation task [previous studies].

% Conversational AI에 대한 수요가 급부상함에 따라, CRS를 통한 아이템 추천에 대한 연구가 큰 관심을 받고 있다.
% Conversational Recommdner Systems(CRS)는 사용자와의 실시간 상호작용을 통해 사용자의 맥락과 요구를 심도 있게 이해함으로써 맞춤형 추천을 제공하는 것을 목표로 한다.

% 2. 기존 연구의 두 갈래 방향 소개 및 한계
Existing CRS는 사용자와 시스템 간의 대화에서 자연어로 표현된 선호도를 파악하고, 추천 도메인의 지식을 활용하여 고품질의 추천을 제공하는 것을 목표로 한다.
The traditional approaches는 영화 추천을 위해 movie knowledge graph를 external knowledge로 활용하여 부족한 domain-related context information를 보완한다~\cite{crs2019kbrd, crs2020kgsf, crs2021revcore, crs2022unicrs}.
하지만, 이러한 접근법은 대화 내 문맥을 파악하는 데 있어서 entity-level의 도메인 지식만을 활용하는 한계가 있다~\cite{crs2021revcore}. 이를 극복하기 위해, 최신 연구들은 LLM의 방대한 world knowledge와 reasoning ability를 활용하여 recommender 자체로 활용하는 방법을 탐구하고 있다.
그럼에도 불구하고 이러한 두 방향 모두 새로운 도메인이나 아이템을 활용하는 데에 제약이 있다. Knowledge graph는 본질적으로 새로운 entity나 relation 추가가 어려우며 구축이 비싸다. LLM의 경우 사전에 학습된 지식에 의존하므로, 실시간으로 변화하는 정보나 새로운 지식을 반영하는 데 제약이 있으며 고정된 popular items을 반복적으로 추천한다는 문제가 지적된다~\cite{survey/crs2024userstudy, survey/crs2023llmfair}. 이는 사용자 만족도를 저하시킨다.

% 또 다른 갈래로, Large Language Models(LLM)을 활용한 최근의 연구들은 LLM을 recommender itself로 활용하는 방향으로, 방대한 world knowledge와 reasoning ability를 기반으로 뛰어난 잠재력을 보이고 있다\cite{crs2024chatcrs,crs2023llmzs}. 
% 하지만 이러한 두 방향은 모두 새로운 도메인과 새로운 아이템에 제약이 있다는 한계가 있다.
% 먼저 KG 기반 model들은 KG에 의존적이며, KG가 구축되기 어려운 환경에서는 동작할 수 없다는 한계를 보인다.
% 또한 LLM은 전에 학습된 지식이 고정되어 있어, 실시간으로 변화하는 정보나 새로운 지식을 즉각적으로 반영하는 데 있어 근본적인 제약을 가지고 있다.
% 새로운 아이템이나 pre-trained corpera에 많이 등장하지 않은 cold 도메인에 관한 지식을 처리할 때 LLM만으로는 충분히 대응하기 어려우며, LLM의 internally 부족한 knowledge에 대해서는 높은 품질의 추천을 제공할 수 없다.

% 2. [kook]
% CRS는 사용자와의 상호작용을 통해 자연어로 표현된 preference를 이해하고, 도메인 지식을 활용하여 적절한 추천을 제공하는 것을 목표로 한다. Traditional CRS는 특히 영화 추천 분야에서, 대화 내 부족한 domain knowledge를 보완하기 위해 knowledge graph를 external knowledge로 활용하는 데 중점을 둔다. 이러한 방법은 영화와 관련된 다양한 entity (e.g., actor, director, genre, etc.)와 그들 간의 복잡한 관계를 정교하게 모델링하여 대화 내 언급된 entities를 기반으로 정확한 추천을 가능하게 한다.
% 하지만 KG-based 모델은 주로 word-level 및 entity-level의 knowledge graph를 사용하기 때문에 문맥을 완전히 고려하는 데 한계가 있다. 이러한 한계를 하결하기 위해 최근 연구에서는 LLM을 recommender itself로 활용하는 방안이 최근 많이 탐구되고 있다. LLM은 world knowledge와 reasoning ability를 바탕으로 뛰어난 성능과 잠재력을 보여주고 있다. 또한, ChatCRS에서는 knowledge graph를 활용하여 외부 지식을 보강함으로써 KG-based와 LLM-based 기반 접근 방식이 가진 한계를 극복하려는 시도도 있다.
% 하지만, 이러한 두 접근 방식 모두 새로운 도메인이나 새로운 아이템을 다룰 떄 제약이 있다는 한계가 있다. 지식 그래프와 LLM은 도메인 지식을 효과적으로 전달하는 역할을 수행할 수 있지만, KG는 새로운 concept이나 relation을 추가하는 것이 어렵다는 본질적인 한계가 존재한다. 또한, LLM은 사전 학습된 지식이 쉽게 outdated될 수 있으며, 최신 지식이나 새로운 아이템에 대한 확장성이 낮다는 문제가 있다. 
% -> new item에 대한 확장성을 retrieval-based method의 당위성으로 연결결

% 3. Retrieval-based의 당위성
최근 연구~\cite{crsret2023CRSRetbaseline}에서는 위 challenges를 해결하기 위해 retrieval-based CRS를 제안한다. 이는 CRS task를 information retrieval (IR) task로 reformulate하여, 주어진 conversation (query)에 부합하는 item (document)를 찾는 것을 목표로 한다.
% 구체적으로,~\citet{crsret2023CRSRetbaseline}는 BM25와 user-centric modeling을 사용하여 새로운 아이템에 대한 추가적인 모델 학습 없이도 추천이 가능함을 보인다.
Retrieval-based CRS는 (i) xx하기 때문에, knowledge graph와 같은 external knowledge의 의존도를 크게 줄이고, (ii) 새로운 아이템에 대한 추가 학습이 필요 없기 때문에, 새로운 아이템에 대한 높은 확장성을 지닌다.

% 3. [kook]
% 최근 연구는 retrieval-based CRS를 제안하였다. 이 접근 방식은 CRS 문제를 information retrieval(IR) task로 재정의하여, 주어진 conversation(query)에 item(docu,emt)를 찾는 것을 목표로 한다. 구체적으로, \cite{largegupta}는 BM25와 user-centric modeling을 통해 새로운 아이템에 대한 추가적인 모델 학습 없이도 추천이 가능함을 보인다. 이러한 방식은 KG와 같은 external knowledge에 대한 의존도를 크게 줄이며, 아이템 메타 데이터를 활용하여 새로운 아이템에 대한 높은 확장성을 지닌다. 


%(MESE, PECRS보고 보충)
% 4. IR 방식의 한계
하지만 기존 연구는 query와 conversation의 차이를 간과함으로써 몇 가지 한계를 드러내었다.
(i) Queries in CRS may involve ambiquities하며 사용자의 선호는 implicit하고 context dependent하다.
일반적인 IR의 쿼리는 문맥 추론이 요구되지 않는 straightforward한 phrase인 반면, conversation은 previous turn, 대화 내 underlying needs and implicitly expressed preferences를 파악해야 한다. 또한, 사용자에게 가장 관련된 아이템을 추천하기 위해 potential preferences를 추론하는 것이 중요하다.
따라서, CRS 문제를 IR과 같은 방식으로 해결하는 것은 위와 같은 중요한 차이를 간과할 수 있다.
% (i) Query는 명시적 정보만 포함하지만 Conv.는 암시적 의도가 담겨 있다.
% Query에는 문맥 추론이 필요하지 않은 straightforward한 phrase이다.
% Conv.(\eg Do you seriously think that movie is fun?)는 대화의 맥락과 암시적 의도를 파악해야 한다.
% 따라서, CRS 문제를 IR과 같은 방식으로 해결하는 것은 위와 같은 중요한 차이를 간과할 수 있다.

(ii) 검색 시 사용자의 상반되는 긍정/부정에 대한 선호를 고려해야 한다.
사용자의 발화는 단순히 positive preferences만을 반영하는 것이 아니라, 서로 상반된 선호—즉, like와 dislike—를 동시에 나타낼 수 있다.
하지만, Conversation에는 positive preference뿐만 아니라 negative preference 또한 함께 나타나며, 이 두 preference는 검색에서 다르게 해석되어야 한다. 예를 들어, Figure~\ref{fig:motivating}에서 보여지는 바와 같이, 사용자가 “나는 액션 영화를 좋아하지만 폭력적인 장면은 싫어한다”고 말할 경우, 전통적인 IR 시스템은 사용자의 부정적인 선호를 고려하지 않고 잔인한 액션 영화를 추천할 수 있다. 이는 사용자의 상반되는 선호를 모두 같은 의도(가깝게)로 다룬 결과이며, 이는 sub-optimal한 결과로 이어질 수 있다.


% (ii) 선호의 긍/부정에 대한 고려가 필요하다.
% Query에서 언급되는 entity는 잠재적으로 사용자가 like한다고 볼 수 있다.
% 하지만 Conversation에서 사용자는 대화 중 언급되는 item과 attribute에 대해 positive preference뿐만 아니라 negative dislike를 함께 나타낸다.
% 만약 이렇게 서로 다른 preference를 differentiate하지 않는다면, 이는 sub-optimal한 결과로 이어질 수 있다.

% [kook] 그러나, 단순히 IR 방식을 CRS에 적용하는 것은 몇 가지 중요한 한계를 드러낼 수 있다. (i) Traditional IR은 사용자 발화에 multiple intents가 존재할 가능성을 충분히 고려하지 못한다. 사용자의 발화는 단순히 positive preferences만을 반영하는 것이 아니라, 서로 상반된 의도—즉, like와 dislike—를 동시에 나타낼 수 있다. \textbf{예를 들어, Figure 1에서 보여지는 바와 같이(예시 figure 추가),} 사용자가 “나는 액션 영화를 좋아하지만 폭력적인 장면은 싫어한다”고 말할 경우, 전통적인 IR 시스템은 이 발화를 모두 긍정적인 선호를 가진 쿼리 덩어리로 간주하여 잔인한 액션 영화를 추천할 수 있다. 이는 사용자의 복잡한 의도를 제대로 이해하지 못한 결과이며, 이로 인해 부정확한 추천이 이루어져 사용자 만족도를 크게 저하시킬 수 있다.
% [kook] (ii) 사용자의 긍/부정 선호를 고려한 검색 방식이 필요하다.
% 기존 연구에서는 대화 내 언급된 entity의 like/dislike를 고려하지 않는다(ChatCRS, UniCRS, LargeGupta). 사용자의 sentiment polarity를 고려한 연구들이 존재하지만(RevCore, ECR), 이것들을 item search/ranking에 직접적으로 활용하지 않는다. (user representation을 보강하는 용도?) 하지만, 사용자는 대화 중 언급되는 item과 attribute에 대해 positive/negative preference를 함께 언급하며, 이를 단일한 의도를 가진 쿼리로 취급하는 것은 sub-optimal한 결과로 이어질 수 있다(LargeGupta).
% 이러한 한계를 극복하기 위해서는, retrieval-based CRS가 사용자 발화 내에 존재하는 복잡적인 의도를 정확하게 분석하고 이를 검색에 반영할 수 있는 능력이 필요하다. 구체적으로, 발화에서 나타나는 긍정적 의도와 부정적 의도를 명확히 구분하고, 이를 바탕으로 아이템을 차별화된 방식으로 평가하는 접근이 요구된다. 사용자가 긍정적 의도를 나타낸 아이템은 우선적으로 상위에 랭크시키고, 부정적 의도를 포함한 아이템은 하위에 배치하는 방식으로 사용자 선호를 더욱 정밀하게 반영해야 한다. 이러한 방식은 기존 IR 시스템과 차별화된 혁신적인 접근으로, CRS의 추천 성능을 극적으로 향상시킬 수 있다.

% 5. Contribution or LorD
위의 한계들을 다루기 위해, 우리는 대화 내에 존재하는 복잡하고 충돌되는 선호를 정확하게 반영할 수 있는 retrieval-based CRS framework \ours를 제안한다. 모델은 핵심적인 두 가지 절차로 구성된다. (i) Preference reasoning, (ii) Preference-aware learning. 먼저 preference reasoning 단계에서, 우리는 LLM의 reasoning ability를 활용하여 사용자와 시스템 사이의 대화 내 존재하는 혼재되고 암시적인 선호를 like와 dislike로 구분하여 추출하고, 이로부터 추천을 효과적으로 보조할 수 있는 사용자의 potential preference를 추론하여 증강한다. 
Preference-aware learning 단계에서는 서로 상반되는 preference를 직접 학습에 반영함으로써 사용자의 의도에 부합하는 최적의 결과를 검색할 수 있도록 한다.

% 위의 두 한계를 해결하기 위해 우리는 사용자의 복합적인 선호를 효과적으로 반영할 수 있는 retrieval-based CRS framework \ours를 제안한다.
% \ours는 Preference Reasoning과 Preference-aware Learning 크게 두 component로 구성되어 있다.
% 먼저 Preference Reasoning은 Conversation 내의 암시적 의도를 파악하고 사용자 발화 beyond의 선호를 추론할 수 있는 단계이다.
% 구체적으로, it LLM을 활용하여 사용자와 시스템 사이의 대화 내 존재하는 혼재되고 선호를 like와 dislike로 구분해 추출하고, 추출해낸 preference와 대화를 기반으로 LLM의 reasoning 능력을 통해 사용자의 potential preference을 추론한다.
% 두번째로, Preference-aware Learning Framework를 통해 상반된 preference를 구별하여 사용자의 의도를 파악한다. (차별점이 더 드러나도록록 작성하기)
% Moreover, 더 효과적이고, 효율적으로 학습할 수 있는 hard negative sampling을 제안한다.

% [kook] 위 두 한계를 다루기 위해, 본 논문에서는 사용자의 발화 내에 존재하는 복합적인 선호와 의도를 정확하게 분석하고 이를 검색에 반영할 수 있는 simple yet effective한 retrieval-based CRS framework /ours를 제안한다. 
% 구체적으로, 우리는 LLM을 reasoning ability를 활용하여 사용자와 시스템 사이의 대화 내 존재하는 혼재되고 암시적인 선호를 like와 dislike로 정확하게 구분해 추출하고, 이로부터 사용자의 potential preference를 증강하는 방법을 제시한다. 이와 같은 접근은 단순히 대화 내에 표면적으로 드러난 사용자의 선호 뿐만 아니라, 암시적으로 표현된 의미있는 사용자 선호 정보를 도출함으로써 사용자의 선호를 보다 정교하게 이해하고 반영할 수 있다. 또한, 본 연구는 복잡한 사용자 발화 속 상반되는 선호를 효과적으로 학습하고, 이를 scoring에 반영하는 것이 CRS task에 적합함을 실헙적으로 입증한다. 이를 통해, 우리는 기존의 IR-style 방식과 차별화된 학습 방식을 제안한다. 이 방법은 사용자의 선호를 like와 dislike로 나누어 서로 차별적으로 반영하여 가장 관련성이 높은 아이템을 검색하는 데 중점을 두며, CRS의 추천 성능을 극적으로 향상시킬 수 있는 가능성을 보여준다. 더불어, 검색 모델을 더 effective and efficient하게 학습할 수 있는 hard negative sampling을 제안한다.

The main contributions of our work are summarized as follows:

\begin{itemize}
    \item 우리는 LLM reasoning 능력을 활용하여 대화 내에서 자연어로 복잡하게 표현된 선호를 파악하고, 효과적인 추천을 위한 potential preference를 증강하여 사용하며 실험을 통해 생성된 데이터의 효과성을 보인다.
    \item 우리는 대화 내에서 사용자가 나타내는 상반되는 preference를 반영할 수 있는 preference-aware retrieval learning framework를 고안하며, 실험을 통해 그 효과성을 증명한다.
    \item 두개의 dataset에서 \ours가 baseline을 ourperform한 것을 보였고, 다양한 모델에서의 Extensive experiment를 통해 우리의 증강된 preference와 learning framework의 유효성을 보였다. 데이터셋과 코드는 추후 공개할 예정이다.
\end{itemize}


% \begin{itemize}
%     \item 우리는 IR과 CRS의 gap을 bridge하기 위한 retriever-based CRS framework를 제안한다.
%     \item 우리는 LLM reasoning 능력을 활용하여 대화 내에서 자연어로 복잡하게 표현된 선호를 파악하고, 그 너머에 있는 사용자의 선호를 추론하였다. -> recommendation을 위한 사용자의 potential preference를 추출하여 성능을 개선했다는 점...
%     \item 우리는 preference-aware retrieval learning framework를 통해 대화 내에서 사용자가 나타내는 상반되는 prefernece를 구분하여 추천하였다.
%     \item 두개의 dataset에서 \ours가 baseline을 ourperform한 것을 보였고, 다양한 모델에서의 Extensive experiment를 통해 우리의 증강된 preference와 learning framework의 유효성을 보였다. 데이터셋과 코드는 추후 공개할 예정이다.
% \end{itemize}

% \item \textbf{Utilizing LLM reasoning to enhance preference extraction and augmentation:} We utilize the reasoning capabilities of LLMs to extract user preferences from dialogues and augment potential preferences, demonstrating superior performance even in zero-shot settings. We also plan to release our dataset for public use.
% \item \textbf{Introducing a preference-aware retrieval learning approach:} We propose a retrieval learning strategy that explicitly accounts for conflicting intents within user dialogues. Experimental results on benchmark datasets showcase the superiority of our approach over existing methods.
% \item \textbf{Expanding the scope of retrieval-based CRS research:} We establish a novel methodology that differentiates itself by focusing exclusively on enhancing recommendation quality, rather than on general text generation, which LLMs already excel at. Our method redefines query generation, learning processes, and scoring strategies to optimize retrieval-based CRS efficiency.

% 본 연구는 LLM이 이미 성공적으로 수행하는 텍스트 생성 작업을 제외하고, 철저하게 추천에 집중한다. 우리는 IR 방식과는 차별화된 쿼리 생성, 학습, 점수 계산 방식을 제안하여, retrieval-based CRS의 효율성을 한층 더 끌어올릴 것이다. 우리의 접근 방식은 간단하면서도 강력하며, 여러 실험을 통해 그 효과를 입증하였다. 마지막으로, 우리는 공식 코드와 다양한 데이터셋을 공개할 것이다.

==> body/backup/1_introduction_backup241010.tex <==
\input{figures/figures_tex/fig_motivating}
\section{Introduction}
\label{sec:introduction}

% % 1. CRS 설명, 두 가지 Task 설명
% % 2. 기존 CRS 소개 및 한계점
% %  - 1) KG vs. LLM vs. Retrieval-based CRS
% %  - 2) emotion-aware vs. non-emotion-aware
% % 3. Retriever CRS (위 두 방법 대비 어떤 장점이 있는지)
% % 4. Challenges (하지만 무엇을 해결하지 못했는지)
% % 5. Contribution

% % 1. CRS 설명, 두 가지 task 설명, 기존 방식의 한계 간략하게 언급
% In recent years, Large Language Models (LLMs) have accelerated the advancement of Conversational AI, leading to a growing interest and demand for Conversational Recommender Systems (CRS).
% CRS yields personalized recommendations by deeply understanding the user's context and needs through real-time interactions. It enhances the user's personalized experience by providing recommendations that are more aligned with their preferences and evolving requirements.
In recent years, Large Language Models (LLMs) have accelerated the advancement of Conversational AI, leading to a growing interest and demand for Conversational Recommender Systems (CRSs).
They yield personalized recommendations by deeply understanding the user's context and needs through real-time interactions and enhance the user experience by providing recommendations that are more aligned with their preferences and evolving requirements.

기존 CRS models은 주로 knowledge graph를 활용하여 대화에서 다루어지는 도메인과 관련된 entity에 대한 지식을 보강함으로써, 부족한 domain-related contextual information을 보완한다. 이러한 접근 방식은 특정 도메인에 대한 지식이 부족할 때 효과적일 수 있는 방법이지만, knowledge graph의 낮은 확장성으로 인해 여전히 제한된 정보만을 활용할 수 있다.
이와 같은 한계를 극복하기 위해 최근에는 LLMs의 뛰어난 문맥 이해 능력과 방대한 world knowledge를 활용하여, LLMs을 recommender 그 자체로 활용하려는 연구가 주목받고 있다. 또한, 부족한 도메인 지식을 external knowledge (\eg, knowledge graph)를 활용하여 LLMs의 근본적인 한계인 lack of specific knowledge를 해결하고자 한다.

그러나 CRS 태스크에서는 단순히 대화에 등장한 엔티티 수준의 정보만을 고려하는 것만으로는 사용자의 진정한 의도와 선호를 충분히 반영하기 어렵다. 사용자의 감정 정보를 배제하고 단순히 엔티티만을 고려하는 접근 방식은 사용자의 복잡한 의도와 맥락을 무시하게 되어, 이는 최적의 결과를 도출하는 데 한계를 초래할 수 있다. 이에 대응하여, 몇몇 연구들은 entity-level에서 사용자의 감정을 세분화하여 고려하는 접근법을 도입한다~\cite{crs2021revcore}. MemoCRS는 LLM을 이용하여 context-level에서 사용자의 선호를 고려하는 attributes를 추출하여 이에 대한 사용자의 태도를 반영하고 reranking을 수행한다.
% RevCore는 entity-level에서 사용자의 선호를 긍정과 부정으로 분류하여, 사용자의 감정 정보를 반영한 리뷰를 검색하여 user representation을 보강한다. ECR은 entity-level에서 9가지의 세분화된 감정을 부여함으로써 사용자의 선호를 더욱 정밀하게 고려하는 추천을 수행한다.


하지만 기존 연구들은 대화 내 존재하는 사용자의 선호를 다루는 데 두 가지 주요 한계를 가지고 있다. (i) 다양한 세부 수준으로 추출된 선호 정보를 추천 시스템과 효과적으로 정렬하지 못한다. 이러한 접근법은 추출된 선호를 단순히 고려하는 데 그치고, 이를 직접적으로 랭킹에 반영하는 학습 방법의 효과를 충분히 활용하지 못하고 있다. (ii) 또한, 기존 연구들은 사용자의 상충되는 선호 정보를 최적화된 방식으로 반영하지 못한다는 문제가 있다. 실제 사용자와 시스템 간의 대화에는 상반된 선호, 예를 들어 like와 dislike가 혼재되어 있으며, 이 선호들은 서로 다른 의도를 나타낸다(\ie, 사용자가 좋아하는 항목은 추천 목록에서 가깝게 배치되고, 싫어하는 항목은 멀리 배치.)

% [feedback] 각 component가 앞의 limitation을 각각 address하는 것으로 매칭되게 하면 좋을 것 같아요 (가능하다면)
본 논문에서는 대화 내 이러한 상반된 선호를 아이템 추천에 최적화된 방식으로 학습하는 것을 목표로 한다. 자연어 정보를 가장 효과적으로 활용할 수 있는 Information retrieval(IR)-style을 채택하였으며, 검색 과정에서 사용자의 like/dislike 정보를 명시적으로 반영하는 simple yet effective한 retrieval-based CRS framework, \ours. 
구체적으로, 우리는 두 가지 핵심 단계를 걸친다, (i) Preference reasoning stage, (ii) Preference-aware alignment learning (가제). Prefernce reasoning stage에서는 주어진 LLM을 reasoning ability를 활용하여 사용자와 시스템 사이의 대화 내 존재하는 혼재되고 암시적인 선호를 like와 dislike로 정확하게 구분해 추출하고, 이로부터 사용자의 potential preference를 증강하는 방법을 제시한다. 이와 같은 접근은 단순히 대화 내에 표면적으로 드러난 사용자의 선호 뿐만 아니라, 잠재적인 선호를 추론해냄으로써 추천에 직접적으로 이러저러하게. Prefernece-aware alignment learning stage에서는 서로 상반되는 사용자의 선호를 또한, 본 연구는 복잡한 사용자 발화 속 상반되는 선호를 효과적으로 학습하고, 이를 scoring에 반영하는 것이 CRS task에 적합함을 실헙적으로 입증한다.

본 연구의 주요 contributions은 아래와 같다:
\begin{itemize}
    \item 흠
    \item 흐음
    \item 세번째
\end{itemize}

본 연구는 최근 LLM의 발전이 자연어 생성에 있어서 naturalness를 향상시켰기에, 사용자의 선호를 aligning하는 것을 심도있게 탐구하기 위해 철저하게 추천에 집중한다.

% % 2. 기존 연구의 두 갈래 방향 소개 및 한계
% % [feedback] 이 문장은 앞 문단에 CRS 설명할때 같이 녹여내는게 좋아보여요. 여기에서는 기존 연구를 갈래를 바로 나누고 각각 설명하는게 어떨까 싶습니다. 예시) Existing CRS models은 xx를 기준으로 KG, LLM, Retrieval-based CRS로 분류된다. (KG 소개) KG-based CRS는 KG를 활용해 xx를 수행한다. (KG 한계점) 하지만, KG-based CRS은 scaliablity에 취약하여 xx하기 어렵다.
% Existing CRS는 사용자와 시스템 간의 대화에서 자연어로 표현된 선호도를 파악하고, 추천 도메인의 지식을 활용하여 고품질의 추천을 제공하는 것을 목표로 한다.
% The traditional approaches는 영화 추천을 위해 movie knowledge graph를 external knowledge로 활용하여 부족한 domain-related context information를 보완한다~\cite{crs2019kbrd, crs2020kgsf, crs2021revcore, crs2022unicrs}. 
% 하지만, 이러한 접근법은 대화 내 문맥을 파악하는 데 있어서 entity-level의 도메인 지식만을 활용하는 한계가 있다. 이를 극복하기 위해, 최신 연구들은 LLM의 방대한 world knowledge와 reasoning ability를 활용하여 recommender 자체로 활용하는 방법을 탐구하고 있다.
% 그럼에도 불구하고 이러한 두 방향 모두 새로운 도메인이나 아이템을 활용하는 데에 제약이 있다. Knowledge graph는 본질적으로 새로운 entity나 relation 추가가 어려우며 구축이 비싸다. LLM의 경우 사전에 학습된 지식에 의존하므로, 실시간으로 변화하는 정보나 새로운 지식을 반영하는 데 제약이 있으며 고정된 popular items을 반복적으로 추천한다는 문제가 지적된다~\cite{survey/crs2024userstudy, survey/crs2023llmfair}. 

% 몇몇 연구들은 대화 내 언급된 entity에 대한 사용자의 감정을 고려하여 사용자 표현을 향


% % 3. Retrieval-based의 당위성
% % [feedback] retrieval-based 연구가 gupta 하나라면, 이 문장은 위에 합쳐도 될 것 같아요. (구체적으로~) 이렇게 들어가지 않아도 될 것 같아서요 ㅎㅎ
% % 최근 연구~\cite{crsret2023CRSRetbaseline}에서는 위 challenges를 해결하기 위해 retrieval-based CRS를 제안한다. 이는 CRS task를 information retrieval (IR) task로 reformulate하여, 주어진 conversation (query)에 부합하는 item (document)를 찾는 것을 목표로 한다.
% % Retrieval-based CRS는 (i) xx하기 때문에, knowledge graph와 같은 external knowledge의 의존도를 크게 줄이고, (ii) 새로운 아이템에 대한 추가 학습이 필요 없기 때문에, 새로운 아이템에 대한 높은 확장성을 지닌다.


% % (ii) 선호의 긍/부정에 대한 고려가 필요하다.
% % Query에서 언급되는 entity는 잠재적으로 사용자가 like한다고 볼 수 있다.
% % 하지만 Conversation에서 사용자는 대화 중 언급되는 item과 attribute에 대해 positive preference뿐만 아니라 negative dislike를 함께 나타낸다.
% % 만약 이렇게 서로 다른 preference를 differentiate하지 않는다면, 이는 sub-optimal한 결과로 이어질 수 있다.

% % [kook] 그러나, 단순히 IR 방식을 CRS에 적용하는 것은 몇 가지 중요한 한계를 드러낼 수 있다. (i) Traditional IR은 사용자 발화에 multiple intents가 존재할 가능성을 충분히 고려하지 못한다. 사용자의 발화는 단순히 positive preferences만을 반영하는 것이 아니라, 서로 상반된 의도—즉, like와 dislike—를 동시에 나타낼 수 있다. \textbf{예를 들어, Figure 1에서 보여지는 바와 같이(예시 figure 추가),} 사용자가 “나는 액션 영화를 좋아하지만 폭력적인 장면은 싫어한다”고 말할 경우, 전통적인 IR 시스템은 이 발화를 모두 긍정적인 선호를 가진 쿼리 덩어리로 간주하여 잔인한 액션 영화를 추천할 수 있다. 이는 사용자의 복잡한 의도를 제대로 이해하지 못한 결과이며, 이로 인해 부정확한 추천이 이루어져 사용자 만족도를 크게 저하시킬 수 있다.
% % [kook] (ii) 사용자의 긍/부정 선호를 고려한 검색 방식이 필요하다.
% % 기존 연구에서는 대화 내 언급된 entity의 like/dislike를 고려하지 않는다(ChatCRS, UniCRS, LargeGupta). 사용자의 sentiment polarity를 고려한 연구들이 존재하지만(RevCore, ECR), 이것들을 item search/ranking에 직접적으로 활용하지 않는다. (user representation을 보강하는 용도?) 하지만, 사용자는 대화 중 언급되는 item과 attribute에 대해 positive/negative preference를 함께 언급하며, 이를 단일한 의도를 가진 쿼리로 취급하는 것은 sub-optimal한 결과로 이어질 수 있다(LargeGupta).
% % 이러한 한계를 극복하기 위해서는, retrieval-based CRS가 사용자 발화 내에 존재하는 복잡적인 의도를 정확하게 분석하고 이를 검색에 반영할 수 있는 능력이 필요하다. 구체적으로, 발화에서 나타나는 긍정적 의도와 부정적 의도를 명확히 구분하고, 이를 바탕으로 아이템을 차별화된 방식으로 평가하는 접근이 요구된다. 사용자가 긍정적 의도를 나타낸 아이템은 우선적으로 상위에 랭크시키고, 부정적 의도를 포함한 아이템은 하위에 배치하는 방식으로 사용자 선호를 더욱 정밀하게 반영해야 한다. 이러한 방식은 기존 IR 시스템과 차별화된 혁신적인 접근으로, CRS의 추천 성능을 극적으로 향상시킬 수 있다.

% % 5. Contribution or LorD
% 위의 한계들을 다루기 위해, 우리는 대화 내에 존재하는 복잡하고 충돌되는 선호를 정확하게 반영할 수 있는 retrieval-based CRS framework \ours를 제안한다. 모델은 핵심적인 두 가지 절차로 구성된다. (i) Preference reasoning, (ii) Preference-aware learning. 먼저 preference reasoning 단계에서, 우리는 LLM의 reasoning ability를 활용하여 사용자와 시스템 사이의 대화 내 존재하는 혼재되고 암시적인 선호를 like와 dislike로 구분하여 추출하고, 이로부터 추천을 효과적으로 보조할 수 있는 사용자의 potential preference를 추론하여 증강한다. 
% Preference-aware learning 단계에서는 서로 상반되는 preference를 직접 학습에 반영함으로써 사용자의 의도에 부합하는 최적의 결과를 검색할 수 있도록 한다.

% % 위의 두 한계를 해결하기 위해 우리는 사용자의 복합적인 선호를 효과적으로 반영할 수 있는 retrieval-based CRS framework \ours를 제안한다.
% % \ours는 Preference Reasoning과 Preference-aware Learning 크게 두 component로 구성되어 있다.
% % 먼저 Preference Reasoning은 Conversation 내의 암시적 의도를 파악하고 사용자 발화 beyond의 선호를 추론할 수 있는 단계이다.
% % 구체적으로, it LLM을 활용하여 사용자와 시스템 사이의 대화 내 존재하는 혼재되고 선호를 like와 dislike로 구분해 추출하고, 추출해낸 preference와 대화를 기반으로 LLM의 reasoning 능력을 통해 사용자의 potential preference을 추론한다.
% % 두번째로, Preference-aware Learning Framework를 통해 상반된 preference를 구별하여 사용자의 의도를 파악한다. (차별점이 더 드러나도록록 작성하기)
% % Moreover, 더 효과적이고, 효율적으로 학습할 수 있는 hard negative sampling을 제안한다.

% % [kook] 위 두 한계를 다루기 위해, 본 논문에서는 사용자의 발화 내에 존재하는 복합적인 선호와 의도를 정확하게 분석하고 이를 검색에 반영할 수 있는 simple yet effective한 retrieval-based CRS framework /ours를 제안한다. 
% % 구체적으로, 우리는 LLM을 reasoning ability를 활용하여 사용자와 시스템 사이의 대화 내 존재하는 혼재되고 암시적인 선호를 like와 dislike로 정확하게 구분해 추출하고, 이로부터 사용자의 potential preference를 증강하는 방법을 제시한다. 이와 같은 접근은 단순히 대화 내에 표면적으로 드러난 사용자의 선호 뿐만 아니라, 암시적으로 표현된 의미있는 사용자 선호 정보를 도출함으로써 사용자의 선호를 보다 정교하게 이해하고 반영할 수 있다. 또한, 본 연구는 복잡한 사용자 발화 속 상반되는 선호를 효과적으로 학습하고, 이를 scoring에 반영하는 것이 CRS task에 적합함을 실헙적으로 입증한다. 이를 통해, 우리는 기존의 IR-style 방식과 차별화된 학습 방식을 제안한다. 이 방법은 사용자의 선호를 like와 dislike로 나누어 서로 차별적으로 반영하여 가장 관련성이 높은 아이템을 검색하는 데 중점을 두며, CRS의 추천 성능을 극적으로 향상시킬 수 있는 가능성을 보여준다. 더불어, 검색 모델을 더 effective and efficient하게 학습할 수 있는 hard negative sampling을 제안한다.

% The main contributions of our work are summarized as follows:

% \begin{itemize}
%     \item 우리는 LLM reasoning 능력을 활용하여 대화 내에서 자연어로 복잡하게 표현된 선호를 파악하고, 효과적인 추천을 위한 potential preference를 증강하여 사용하며 실험을 통해 생성된 데이터의 효과성을 보인다.
%     \item 우리는 대화 내에서 사용자가 나타내는 상반되는 preference를 반영할 수 있는 preference-aware retrieval learning framework를 고안하며, 실험을 통해 그 효과성을 증명한다.
%     \item 두개의 dataset에서 \ours가 baseline을 ourperform한 것을 보였고, 다양한 모델에서의 Extensive experiment를 통해 우리의 증강된 preference와 learning framework의 유효성을 보였다. 데이터셋과 코드는 추후 공개할 예정이다.
% \end{itemize}


% % \begin{itemize}
% %     \item 우리는 IR과 CRS의 gap을 bridge하기 위한 retriever-based CRS framework를 제안한다.
% %     \item 우리는 LLM reasoning 능력을 활용하여 대화 내에서 자연어로 복잡하게 표현된 선호를 파악하고, 그 너머에 있는 사용자의 선호를 추론하였다. -> recommendation을 위한 사용자의 potential preference를 추출하여 성능을 개선했다는 점...
% %     \item 우리는 preference-aware retrieval learning framework를 통해 대화 내에서 사용자가 나타내는 상반되는 prefernece를 구분하여 추천하였다.
% %     \item 두개의 dataset에서 \ours가 baseline을 ourperform한 것을 보였고, 다양한 모델에서의 Extensive experiment를 통해 우리의 증강된 preference와 learning framework의 유효성을 보였다. 데이터셋과 코드는 추후 공개할 예정이다.
% % \end{itemize}

% % \item \textbf{Utilizing LLM reasoning to enhance preference extraction and augmentation:} We utilize the reasoning capabilities of LLMs to extract user preferences from dialogues and augment potential preferences, demonstrating superior performance even in zero-shot settings. We also plan to release our dataset for public use.
% % \item \textbf{Introducing a preference-aware retrieval learning approach:} We propose a retrieval learning strategy that explicitly accounts for conflicting intents within user dialogues. Experimental results on benchmark datasets showcase the superiority of our approach over existing methods.
% % \item \textbf{Expanding the scope of retrieval-based CRS research:} We establish a novel methodology that differentiates itself by focusing exclusively on enhancing recommendation quality, rather than on general text generation, which LLMs already excel at. Our method redefines query generation, learning processes, and scoring strategies to optimize retrieval-based CRS efficiency.

% % 본 연구는 LLM이 이미 성공적으로 수행하는 텍스트 생성 작업을 제외하고, 철저하게 추천에 집중한다. 우리는 IR 방식과는 차별화된 쿼리 생성, 학습, 점수 계산 방식을 제안하여, retrieval-based CRS의 효율성을 한층 더 끌어올릴 것이다. 우리의 접근 방식은 간단하면서도 강력하며, 여러 실험을 통해 그 효과를 입증하였다. 마지막으로, 우리는 공식 코드와 다양한 데이터셋을 공개할 것이다.

==> body/backup/1_introduction_backup241011.tex <==
\input{figures/figures_tex/fig_motivating}
\section{Introduction}
\label{sec:introduction}

%% 1. CRS 설명, 두 가지 Task 설명
%% 2. 기존 CRS 모델 소개 및 한계점 / Retrieval-based CRS 장점
%% 3. Retrieval-based CRSs의 한계점 및 Preference-aware CRSs의 필요성
%% 4. Generation-based models을 사용하는 preference-aware models 소개 및 한계점
%% 5. 위 한계점을 극복하는 제안 방법 소개
%% 6. Contribution


%% 1. CRS 설명 (multi-turn 단어 넣고 싶다)
%In recent years, Large Language Models (LLMs) have accelerated the advancement of Conversational Recommender Systems (CRSs).
Recent advancements in natural language understanding have accelerated the development of Conversational Recommender Systems (CRSs). CRS models deliver personalized recommendations by deeply understanding users' evolving contexts through real-time interactions. Typically, CRSs consist of the following two tasks: \emph{recommendation task} to provide items by identifying the user's intent from the text, and \emph{generation task} to offer a human-friendly response to the user. This paper focuses on the recommendation task rather than the generation task, as recent LLMs have shown impressive naturalness of natural language generation~\cite{}.


%% 2. 기존 CRS 모델 소개 및 한계점 / Retrieval-based CRS 장점
Most CRS approaches \cite{CRS2019KBRD, CRS2020KGSF, CRS2021REVCORE, CRS2022UNICRS} employ generation-based models as recommenders. However, they are limited in reflecting time-varying information or new knowledge, resulting in poor scalability for new items.
% 고정된 popular items을 반복적으로 추천한다는 문제가 있다~\cite{survey/crs2024userstudy, survey/crs2023llmfair}.
To address this issue, a recent work~\cite{crsret2023CRSRetbaseline} introduces a retrieval-based CRS framework. It reformulates the CRS task into an information retrieval (IR) task, which aims to discover items (documents) that correspond to a given conversation (query). Thus, retrieval-based CRSs offer the advantage that new items can be easily added to the candidate pool, requiring no additional training for those items.

% 결과적으로, Retrieval-based CRSs는 새로운 item을 item candidate pool에 쉽게 추가할 수 있기 때문에, the item에 대한 추가 학습이 필요 없다는 장점을 갖는다.
% (ii) xx하기 때문에, external knowledge (\eg, knowledge graph)의 의존도를 크게 줄일 수 있다.


%% 3. Retrieval-based CRSs의 한계점 및 Preference-aware CRSs의 필요성
Although retrieval-based CRSs~\cite{crsret2023CRSRetbaseline} have these advantages, they overlook the intrinsic differences between queries in IR and conversations in CRSs. Generally, IR의 쿼리는 positive 의미를 갖는 straightforward phrase인 반면, conversation은 user preference에 positive와 negative 의미가 혼재할 수 있다~\cite{}. (예시 문장을 가지고 설명하기)

% 예를 들어, Figure~\ref{fig:motivating}에서 보여지는 바와 같이, 사용자가 “나는 액션 영화를 좋아하지만 폭력적인 장면은 싫어한다”고 말할 경우, 전통적인 IR 시스템은 사용자의 부정적인 선호를 고려하지 않고 잔인한 액션 영화를 추천할 수 있다. 이는 사용자의 상반되는 선호를 모두 같은 의도(가깝게)로 다룬 결과이며, 이는 사용자의 의도를 해칠 수 있다.


%% 4. Generation-based models을 사용하는 preference-aware models 소개 및 한계점
\sm{(이 문단에 기존 모델과의 차별성을 보여줄 수 있는 그림 넣기: 희진이가 그린 그림)
이와 관련하여 a few generation-based CRS models~\cite{crs2021revcore} (ECR, MemoCRS 추가)은 conversation 내 user preference 추출을 시도한다. 하지만, 이들은 user-side preference만을 고려하여 xx할 수 없다는 한계가 있다. (여기서 말하는 user-side preference이 무엇인지 설명) 예를 들어,~\cite{crs2021revcore}은 xx하고,~\cite{}는 xx한다. 이들은 user에 conversation 내 언급된 keyphrases 또는 concept과의 관계를 반영하고, item는 학습을 통해 간접적으로 고려하기 때문에 suboptimal에 빠질 수 있다. }


%% 5. 위 한계점을 극복하는 제안 방법 소개
% 우리는 user/item-side preference를 모두 고려하고, 이들을 user와 item representation 사이의 bridge로 활용하여 retreiver를 학습한다. 
In this paper, we propose a novel retrieval-based CRS framework \ours~that extracts and learns user preferences, bridging the gap between IR and CRSs. The proposed \ours~has two key components. (i) \emph{Preference extraction}은 LLMs의 뛰어난 reasoning ability를 활용하여 user와 system 사이의 대화 내 존재하는 암시적인 preference를 positive preference (\ie, \emph{like})와 negative preference (\ie, \emph{dislike})로 정확하게 구분해 추출한다. 그 다음, 추출한 preference를 recommendation task에 맞게 증강하여 사용자의 potential preference를 표현한다.
(ii) \emph{Preference-aware alignment}은 상반된 두 가지의 potential preference를 매개체로 활용하여 recommenders의 효과적인 학습을 수행한다. 구체적으로, positive preference와는 user와 item을 가깝게 학습하고, negative preference와는 user와 item을 멀어지게 학습한다. 이를 통해, recommended item ranking/scoring에 직접적으로 두 가지의 preference를 반영할 수 있으며, xx할 수 있다. Futhermore, 우리는 recommender로 retriever를 사용하기 때문에, alignment learning을 하기에 적합하다.


% preference augmentation 관련 내용 보충 필요
% 하지만 기존 연구들은 대화 내 존재하는 사용자의 선호를 다루는 데 두 가지 주요 한계를 가지고 있다. (i) 다양한 세부 수준으로 추출된 선호 정보를 추천 시스템과 효과적으로 정렬하지 못한다. 이러한 접근법은 추출된 선호를 단순히 고려하는 데 그치고, 이를 직접적으로 랭킹에 반영하는 학습 방법의 효과를 충분히 활용하지 못하고 있다. (ii) 또한, 기존 연구들은 사용자의 상충되는 선호 정보를 최적화된 방식으로 반영하지 못한다는 문제가 있다. 실제 사용자와 시스템 간의 대화에는 상반된 선호, 예를 들어 like와 dislike가 혼재되어 있으며, 이 선호들은 서로 다른 의도를 나타낸다(\ie, 사용자가 좋아하는 항목은 추천 목록에서 가깝게 배치되고, 싫어하는 항목은 멀리 배치.)


The main contributions of our work are summarized as follows:
\begin{itemize}[leftmargin=5mm]
    \item \textbf{Recommendation-tailored Augmentation}: 우리는 IR과 CRS의 gap을 bridge하기 위한 user preference를 추출한다. LLMs의 reasoning 능력을 활용하여 conversation 내에서 natural language로 복잡하게 표현된 선호를 파악하고, recommendation task에 특화된 prompt를 활용해 potential preference를 증강한다.
    \item \textbf{Preference-Recommender Alignment}: 기본적으로, 추출한 preference와 recommenders는 semantic gap이 존재하기 때문에, gap을 완화하기 위해 이들 간 alignment를 실시한다. Aligned recommenders를 활용하여 user preference에 기반한 item 추천을 수행할 수 있다.
    \item \textbf{Comprehensive Validation}: 세 가지의 datasets에서 4종류 7개의 모델들을 outperform한다. Notably, xx 데이터셋에서 최대 xx\%의 performance gain을 보인다. \sm{언급할 만한 추가 실험 언급하기} 실험 xx를 통해 제안 방법의 각 component의 유효성을 보인다.
\end{itemize}


% \begin{itemize}
%     \item 우리는 LLM reasoning 능력을 활용하여 대화 내에서 자연어로 복잡하게 표현된 선호를 파악하고, 효과적인 추천을 위한 potential preference를 증강하여 사용하며 실험을 통해 생성된 데이터의 효과성을 보인다.
%     \item 우리는 대화 내에서 사용자가 나타내는 상반되는 preference를 반영할 수 있는 preference-aware retrieval learning framework를 고안하며, 실험을 통해 그 효과성을 증명한다.
%     \item 두개의 dataset에서 \ours가 baseline을 ourperform한 것을 보였고, 다양한 모델에서의 Extensive experiment를 통해 우리의 증강된 preference와 learning framework의 유효성을 보였다. 데이터셋과 코드는 추후 공개할 예정이다.
% \end{itemize}


% % \begin{itemize}
% %     \item 우리는 IR과 CRS의 gap을 bridge하기 위한 retriever-based CRS framework를 제안한다.
% %     \item 우리는 LLM reasoning 능력을 활용하여 대화 내에서 자연어로 복잡하게 표현된 선호를 파악하고, 그 너머에 있는 사용자의 선호를 추론하였다. -> recommendation을 위한 사용자의 potential preference를 추출하여 성능을 개선했다는 점...
% %     \item 우리는 preference-aware retrieval learning framework를 통해 대화 내에서 사용자가 나타내는 상반되는 prefernece를 구분하여 추천하였다.
% %     \item 두개의 dataset에서 \ours가 baseline을 ourperform한 것을 보였고, 다양한 모델에서의 Extensive experiment를 통해 우리의 증강된 preference와 learning framework의 유효성을 보였다. 데이터셋과 코드는 추후 공개할 예정이다.
% % \end{itemize}

% % \item \textbf{Utilizing LLM reasoning to enhance preference extraction and augmentation:} We utilize the reasoning capabilities of LLMs to extract user preferences from dialogues and augment potential preferences, demonstrating superior performance even in zero-shot settings. We also plan to release our dataset for public use.
% % \item \textbf{Introducing a preference-aware retrieval learning approach:} We propose a retrieval learning strategy that explicitly accounts for conflicting intents within user dialogues. Experimental results on benchmark datasets showcase the superiority of our approach over existing methods.
% % \item \textbf{Expanding the scope of retrieval-based CRS research:} We establish a novel methodology that differentiates itself by focusing exclusively on enhancing recommendation quality, rather than on general text generation, which LLMs already excel at. Our method redefines query generation, learning processes, and scoring strategies to optimize retrieval-based CRS efficiency.


==> body/backup/1_introduction_backup241013.tex <==
\input{figures/figures_tex/fig_motivating}
\section{Introduction}
\label{sec:introduction}

%% 1. CRS 설명, 두 가지 Task 설명
%% 2. Traditional CRS 모델 소개 및 한계점 / Preference-aware CRS 모델 언급
%% 3. Existing Preference-aware CRS 모델 소개 및 한계점
%% 4. 두 가지 Question 던지기
%%    4-1. Q1: 사용자가 좋아하고 싫어하는걸 어떻게 알거고, 이걸 어떻게 표현할거임? (how to represent)
%%    4-2. Q2: 사용자가 좋아하고 싫어하는 걸 어떻게 item과 align해서 추천할거임? (how to align)
%% 5. 제안 방법 소개
%%    5-1. A1: 추출하고 증강하고 text로 표현 (semantic, context 키워드 강점)
%%    5-2. A2: representation learning (user <-> positive preference and negative preference <-> item)
%%         - retrieval-based CRSs의 이점 언급
%% 6. Contribution


%% 1. CRS 설명 (multi-turn 단어 넣고 싶다)
Recent advancements in natural language understanding have accelerated the development of Conversational Recommender Systems (CRSs). CRS models~\cite{pref/crs2021revcore, kg/crs2022unicrs, pref/crs2024ecr, llm/crs2024chatcrs} deliver personalized recommendations by deeply understanding users' evolving contexts through real-time interactions. Typically, CRSs consist of the following two tasks: \emph{recommendation task} to provide items by identifying the user's intent from the text, and \emph{generation task} to offer a human-friendly response to the user. This paper focuses on the recommendation task rather than the generation task, as recent LLMs have shown impressive naturalness of natural language generation~\cite{llm/crs2023llmzs, agent/crs2024interecagent}.


%% 2. 기존 CRS 모델 소개 및 한계점 / Preference-aware CRS 모델 언급
% 한계점: (일단 ECR 한계점으로 적어보기)
Existing CRS approaches~\cite{kg/crs2019kbrd, kg/crs2020kgsf, kg/crs2022unicrs}은 external information (\eg, knowledge graph)나 LLMs의 reasoning 능력을 활용하여 dialogue context를 이해하고, user가 선호할만한 items을 추천한다. 이들은 conversation에 언급된 entity들이 positive하다고만 여긴다. 하지만, user conversation에는 positive와 negative 의미가 혼재하며, human decision-making 과정에서 user sentiment/emotion를 포착하는 것은 user preference modeling함에 있어 중요하다~\cite{lerner2015emotion, pref/crs2024ecr}.


%% 3. Existing Preference-aware CRS 모델 소개 및 한계점 (Motivated Figure)
To address this issue, recent preference-aware CRS models~\cite{pref/crs2021revcore, pref/crs2024ecr, llm/crs2024memocrs}은 conversation 내 user preference를 여러 개의 sentiment/emotion으로 추출하고, 이를 활용하여 정밀한 item recommendation을 수행한다. A literature~\cite{pref/crs2024ecr}은 user utterance 별 9개의 preference label에 대한 확률을 구하고, preference 확률을 하나의 user embedding에 통합시킨다.
However, 이들은 추출한 서로 다른 preference를 다시 user에 통합시킴으로써 user/item와 preference 간의 관계를 학습시켜주지 못 한다, as illustrated in Figure~\ref{fig:motivating}(a).
이러한 예시는 (1) 서로 다른 preference를 differentiate 해야 하며, (2) user-preference 관계뿐만 아니라 user-preference-item 간의 관계를 align해야 한다는 것을 보여준다.
% [준영]
% 또한 사용자의 negative preference와 item의 관계를 학습하지 못한다. (가까워지게만 하고 멀어지는 학습은 하지 못함
% 기존 preference-aware CRS models의 user/item와 preference 학습 방식을 보여준다. 


% However, they are limited in reflecting time-varying information or new knowledge, resulting in poor scalability for new items~\cite{pref/crs2024ecr}.
% 고정된 popular items을 반복적으로 추천한다는 문제가 있다~\cite{survey/crs2024userstudy, survey/crs2023llmfair}.

% To address this issue, a recent work~\cite{ret/crs2023CRSRetbaseline} introduces a retrieval-based CRS framework. It reformulates the CRS task into an information retrieval (IR) task, which aims to discover items (documents) that correspond to a given conversation (query). Thus, retrieval-based CRSs offer the advantage that new items can be easily added to the candidate pool, requiring no additional training for those items.

%% 4. 두 가지 Question 던지기
%%    4-1. Q1: 사용자가 좋아하고 싫어하는걸 어떻게 알거고, 이걸 어떻게 표현할거임?
%%    4-2. Q2: 사용자가 좋아하고 싫어하는 걸 어떻게 item과 align해서 추천할거임?
To this end, we ask the following key questions: \textit{(i) How do we extract dual user preference from the conversation? (ii) How do we learn the relationship between the extracted preference and user/item?}
% [준영]
% (i) How do we extract and represent bilateral user preference from the conversation?
% (ii) How 


%% 5. 제안 방법 소개
%%    5-1. A1: 추출하고 증강하고 text로 표현 (semantic, context 키워드 강점)
%%    5-2. A2: representation learning (user <-> positive preference and negative preference <-> item)
%%         - retrieval-based CRSs의 이점 언급 (Motivated Figure)
To answer the above questions, we propose a novel retrieval-based CRS framework \ours~that extracts and learns user preferences. It has two key components. Firstly, \emph{preference extraction module} leverages the advanced reasoning power of LLMs to accurately distinguish implicit preferences within user-system dialogues into positive (\ie, \emph{like}) and negative (\ie, \emph{dislike}) preferences. Subsequently, the extracted preferences are augmented for the recommendation task to elicit the user's potential preferences.
% Firstly, \emph{Preference extraction module}은 LLMs의 뛰어난 reasoning ability를 활용하여 user와 system 사이의 대화 내 존재하는 암시적인 preference를 positive preference (\ie, \emph{like})와 negative preference (\ie, \emph{dislike})로 정확하게 구분해 추출한다. 그 다음, 추출한 preference를 recommendation task에 맞게 증강하여 사용자의 potential preference를 추론한다.


Secondly, \emph{preference-aware learning module}은 상반된 두 가지의 potential preference를 매개체로 활용하여 recommenders의 효과적인 학습을 수행한다, as depicted in Figure~\ref{fig:motivating}(b). 
우리는 먼저 서로 다른 특징을 가진 conversation, preference, item 간의 관계를 모델링하기 위해 이 세 정보를 모두 text 형태로 표현한 후, dense retriever 구조를 사용하여 모델링한다.
이러한 방식의 이점은 다음과 같다: (i) 모두 같은 모달리티와 모델을 공유해서 같은 representation space에 표현할 수 있고, (ii) 사용자가 같은 preference를 보이는 entity을 LLMs에 통과시켜 general하고 contextual한 표현을 얻을 수 있다.
그 후, [matching]을 통해 positive preference와는 user와 item을 가깝게 학습하고, negative preference와는 user와 item을 멀어지게 학습하며, conv를 사용한 hard negative sampling을 통해 preference를 leverage할 수 있도록 한다
이를 통해, recommended item ranking/scoring에 직접적으로 두 가지의 preference를 반영할 수 있다.
% xx할 수 있다.
% Furthermore, 우리는 recommender로 retriever를 사용하기 때문에, alignment learning을 하기에 적합하다.

% 최근 연구에서는 추천 시스템을 아이템 검색 작업으로 재해석하여, 언어 모델의 semantic understanding과 matching 능력을 극대화하려는 시도가 이루어지고 있다~\cite{ret/rs2024blair, data2024AlignLM2IR, ret/crs2023CRSRetbaseline, ret/crs2024nls}. 사용자의 preference와 item에 대한 preference를 중간 매개체를 효과적으로 활용할 수 있는 건가? 


%% 3. Retrieval-based CRSs의 한계점 및 Preference-aware CRSs의 필요성
% Although retrieval-based CRSs~\cite{ret/crs2023CRSRetbaseline} have these advantages, they overlook the intrinsic differences between queries in IR and conversations in CRSs. Generally, IR의 쿼리는 positive 의미를 갖는 straightforward phrase인 반면, conversation은 user preference에 positive와 negative 의미가 혼재할 수 있다~\cite{}. (예시 문장을 가지고 설명하기)



%% 4. Generation-based models을 사용하는 preference-aware models 소개 및 한계점
% \sm{(이 문단에 기존 모델과의 차별성을 보여줄 수 있는 그림 넣기: 희진이가 그린 그림)
% 이와 관련하여 a few generation-based CRS models~\cite{pref/crs2021revcore} (ECR, MemoCRS 추가)은 conversation 내 user preference 추출을 시도한다. 하지만, 이들은 user-side preference만을 고려하여 xx할 수 없다는 한계가 있다. (여기서 말하는 user-side preference이 무엇인지 설명) 예를 들어,~\cite{pref/crs2021revcore}은 xx하고,~\cite{}는 xx한다. 이들은 user에 conversation 내 언급된 keyphrases 또는 concept과의 관계를 반영하고, item는 학습을 통해 간접적으로 고려하기 때문에 suboptimal에 빠질 수 있다. }



The main contributions of our work are summarized as follows:
\begin{itemize}[leftmargin=5mm]
    \item \textbf{Recommendation-tailored Augmentation}: 우리는 효과적인 user preference modeling을 위해 dual user preference를 추출한다. LLMs의 reasoning 능력을 활용하여 conversation 내에서 natural language로 복잡하게 표현된 preference를 파악하고, recommendation task에 특화된 prompt를 활용해 potential preference를 증강한다.
    \item \textbf{Preference-Recommender Alignment}: 기본적으로, 추출한 preference와 recommenders는 semantic gap이 존재하기 때문에, gap을 완화하기 위해 이들 간 alignment를 실시한다. Aligned recommenders를 활용하여 user preference에 기반한 item 추천을 수행할 수 있다.
    % \item \textbf{Comprehensive Validation}: 세 가지의 datasets에서 4종류 7개의 모델들을 outperform한다. Notably, xx 데이터셋에서 최대 xx\%의 performance gain을 보인다. 실험 xx를 통해 제안 방법의 각 component의 유효성을 보인다. \sm{언급할 만한 추가 실험 언급하기}
    \item \textbf{Comprehensive Validation}: \ours는 세 가지의 datasets에서 4종류의  6개의 모델들을 outperform한다. Notably, CRS에서 많이 사용되는 다양한 preference sparsity를 갖는 세 개의 데이터셋에서 최대 xx\%의 performance gain을 보인다. 특히 ablation study를 통해 like/dislike를 아이템과 분리하여 preference relation을 학습하는  것의 효과적임을 보인다.
    % 특히, LLM을 통해 증강한 user potential preference에 대한 zero-shot 실험을 통해 생성된 데이터가 학습에 유효함을 보인다.

\end{itemize}


% \begin{itemize}
%     \item 우리는 LLM reasoning 능력을 활용하여 대화 내에서 자연어로 복잡하게 표현된 선호를 파악하고, 효과적인 추천을 위한 potential preference를 증강하여 사용하며 실험을 통해 생성된 데이터의 효과성을 보인다.
%     \item 우리는 대화 내에서 사용자가 나타내는 상반되는 preference를 반영할 수 있는 preference-aware retrieval learning framework를 고안하며, 실험을 통해 그 효과성을 증명한다.
%     \item 두개의 dataset에서 \ours가 baseline을 ourperform한 것을 보였고, 다양한 모델에서의 Extensive experiment를 통해 우리의 증강된 preference와 learning framework의 유효성을 보였다. 데이터셋과 코드는 추후 공개할 예정이다.
% \end{itemize}


% % \begin{itemize}
% %     \item 우리는 IR과 CRS의 gap을 bridge하기 위한 retriever-based CRS framework를 제안한다.
% %     \item 우리는 LLM reasoning 능력을 활용하여 대화 내에서 자연어로 복잡하게 표현된 선호를 파악하고, 그 너머에 있는 사용자의 선호를 추론하였다. -> recommendation을 위한 사용자의 potential preference를 추출하여 성능을 개선했다는 점...
% %     \item 우리는 preference-aware retrieval learning framework를 통해 대화 내에서 사용자가 나타내는 상반되는 prefernece를 구분하여 추천하였다.
% %     \item 두개의 dataset에서 \ours가 baseline을 ourperform한 것을 보였고, 다양한 모델에서의 Extensive experiment를 통해 우리의 증강된 preference와 learning framework의 유효성을 보였다. 데이터셋과 코드는 추후 공개할 예정이다.
% % \end{itemize}

% % \item \textbf{Utilizing LLM reasoning to enhance preference extraction and augmentation:} We utilize the reasoning capabilities of LLMs to extract user preferences from dialogues and augment potential preferences, demonstrating superior performance even in zero-shot settings. We also plan to release our dataset for public use.
% % \item \textbf{Introducing a preference-aware retrieval learning approach:} We propose a retrieval learning strategy that explicitly accounts for conflicting intents within user dialogues. Experimental results on benchmark datasets showcase the superiority of our approach over existing methods.
% % \item \textbf{Expanding the scope of retrieval-based CRS research:} We establish a novel methodology that differentiates itself by focusing exclusively on enhancing recommendation quality, rather than on general text generation, which LLMs already excel at. Our method redefines query generation, learning processes, and scoring strategies to optimize retrieval-based CRS efficiency.


==> body/backup/3_model_backup2410152300.tex <==
\input{figures/figures_tex/fig_main}



\section{Proposed Model: \ours} \label{sec:Proposed Method}
This section presents a novel CRS framework \ours, as depicted in Figure~\ref{fig:main}, designed to differentiate between ambivalent user preferences and effectively associate them with items.
% It comprises two components: (i) \emph{ambivalent preference expansion}, which extracts distinct user preferences and infers potential preferences implicitly present in the conversation (Section~\ref{sec:preference_reasoning}); and (ii) \emph{Preference-aware Learning}, which directly models the relationships among the user, ambivalent preferences, and items (Section~\ref{sec:preference_learning}).
% It comprises two components: (i) \emph{ambivalent preference expansion}을 통해 사용자의 서로 다른 선호를 추출하고 대화 내에 대화 내에 함축적으로 포함되어 있는 potential preferences를 추론한다. (Section~\ref{sec:preference_reasoning}) (ii) \emph{preference-aware learning}을 통해 사용자, ambivalent preferences, 그리고 아이템 간의 관계를 직접적으로 모델링한다. (Section~\ref{sec:preference_learning})


% conversation만으로 맞히기 어려운 sample들을 preference를 통해 구분하도록 학습하며 preference 표현을 enhance한다.


% conversation만으로 (어떤 샘플이고 왜 맞히기 힘든데?) 맞히기 어려운 sample들을 preference를 통해 (뭘 구분하도록 하고, 뭐가 optimal한 상태인지) 구분하도록 학습하며 preference 표현을 enhance한다.
% [희진] 모델은 preference signal를 활용하여 conversation만으로는 예측하기 어려운 difficult samples을 구분하도록 학습한다. 이를 통해 사용자가 싫어하는 아이템은 멀게, 좋아하는 아이템은 가깝게 하면서  preference representation을 강화하여 optimal한 matching을 가능하게 하며 추천 정확도를 향상시킨다.

% In this section, 우리는 사용자의 서로 다른 preference를 differentiate하고 item과 align하는 novel CRS framework \ours에 대해 소개한다.
% \ours는 두 component preference reasoning과 preference-aware learning로 구성되어 있다.

% We introduce the two main components of \ours: preference reasoning and preference-aware learning. Fig \ref{fig
% } illustrates the overall framework of \ours. First, we (i) extract and infer different user preferences through recommendation-tailored augmentation (section \ref{sec
% }), and (ii) model the relationships between users, ambivalent preferences, and items through preference-aware learning (section \ref{sec
% }).

\subsection{Ambivalent Preference Expansion}
\label{sec:ambivalent_preference_expansion}
% 기존 연구는 entity 단위로 preference 추출
% 반면 우리는 user의 preference를 text 형태로 추출하여 user와 item 사이의 gap을 bridge하는 역할로 사용함
% \ref{sec:preference_reasoning}을 두 단계로 나눠서 진행: (1) preference를 구분하여 추천하는 것 (2) 대화 beyond의 사용자 preference까지 추론하는 것.
% 기존 연구에서는 대화 내 모든 entity에 대한 preference를 추출한다. 이는 context를 고려하지 않기 때문에 noise한 사용자 선호 정보가 담길 수 있다. 
% 기존 연구에서는 대화 내 등장하는 모든 entity에 대한 사용자의 preference를 추출한다. 하지만, 추출된 entity는 
% 그러나 이 방법은 대화 맥락 내 사용자의 진짜 선호를 충분히 고려하지 않기 때문에, 실제 선호와 관계없는 noise가 포함될 가능성이 있다.
% 우리는 LLM을 이용하여 dialogue history를 고려하여 user's current preferences를 정확하게 추출하고, 이를 기반으로 potential user's preferences를 증강하도록 함으로써 recommendation-assisted augmentation을 수행한다.
We utilize an LLM to analyze the dialogue history and accurately identify the user's current preferences in keyphrase format. Based on these preferences, we prompt the LLM to create several synthetic keyphrases tailored to the user's preferences. The generated keyphrases are used as potential user preferences to assist the retriever in searching for relevant items. Figure ~\ref{fig:main}(a) illustrates this process with an example of conversation.

\subsubsection{User-side Expansion}
\vspace{0.5mm}
\noindent
\textbf{\texttt{Step1}: Current preference extraction.}
For a given user $u$, we integrate the dialogue into a prompt template $P_{\mathrm{ext}}$ as a placeholder and input it into LLMs. We provide a detailed example in the Appendix~\ref{sec:appendix_prompt}.
\begin{equation}
    T_{\mathit{l}}^{\mathrm{ext}}, T_{\mathit{d}}^{\mathrm{ext}} = f_{\mathrm{LLM}}(P_{\mathrm{ext}}, T_c),
\end{equation}
where $T_{\mathit{l}}^{\mathrm{ext}}$ and $T_{\mathit{d}}^{\mathrm{ext}}$ represent lists of keyphrases that capture the positive and negative preferences of user $u$, respectively. By leveraging the reasoning power of LLM, it is possible to analyze the context of dialogue history and accurately extract the user's meaningful surface preferences, allowing for precise distinction between likes and dislikes.

\vspace{0.5mm}
\noindent \textbf{\texttt{Step2}: Potential preference augmentation}. It uses the extracted current preferences of user $u$ to enable the LLM to infer potential preferences that the user might like in the future based on their conversation.
\begin{equation}
    T_{\mathit{l}}^{\mathrm{aug}}, T_{\mathit{d}}^{\mathrm{aug}} = f_{\mathrm{LLM}}(P_{\mathrm{aug}},T_c, T_{\mathit{l}}^{\mathrm{ext}}, T_{\mathit{d}}^{\mathrm{ext}}),
\end{equation}
where $ T_{\mathit{l}}^{\mathrm{aug}} $ and  $T_{\mathit{d}}^{\mathrm{aug}}$ denote lists of keyphrases that infer the potential positive and negative preferences of user $u$, respectively.


\subsubsection{Item-side Expansion}
% \vspace{0.5mm}
% \noindent \textbf{Review summary}.
% 아이템 리뷰는 다수 사용자의 공통된 선호도를 반영하며, 이를 활용해 아이템의 표현력을 강화하고 dense retrieval 기반 접근에서 검색 성능을 높일 수 있다. 특히, dense retrieval에서 주로 사용하는 item metadata는 사용자 preference를 충분히 반영하지 못해 사용자 대화와 아이템 사이의 간극이 발생할 수 있으며, 이를 리뷰의 풍부한 정보로 보완할 수 있다.
% 우리는 IMDb에서 아이템 $i$에 대한 리뷰를 크롤링하고, helpful vote 기준 top $k$개의 리뷰를 수집하였다. 이후 LLM을 사용해 (i) 여러 리뷰에서 공통된 선호도를 추출하여 description으로 요약하고, (ii) 이 description에서 핵심 keyphrase를 뽑아낸다. 이 과정은 redundant 표현을 줄여 표현을 압축하고, 보다 근본적이고 맥락적인 keyphrase로 요약의 품질을 높여 아이템의 표현을 최적화한다.
% Appendix에 이 과정의 구체적인 예시를 포함하여 추가 설명을 제공한다.
% Item reviews reflect the common preferences of many users and can be leveraged to enhance the expressiveness of items, improving search performance in dense retrieval-based approaches. Specifically, the item metadata typically used in dense retrieval may not sufficiently capture user preferences, potentially creating a gap between user conversations and items, which can be bridged by the rich information in reviews.
While users' potential preferences are augmented through LLMs, review summaries can help enhance item expressiveness by filling gaps where metadata lacks detail. Item reviews, reflecting common user preferences, improve search performance in retrieval-based approaches by capturing nuances often missed in item metadata.
% This helps bridge the gap between user conversations and item representation.

% We crawled reviews for item $i$ from IMDb and collected the top $k$ reviews based on helpful votes. We then utilized an LLM to (i) extract common preferences from multiple reviews and summarize them into a description, and (ii) identify key phrases from this description. This process reduces redundant expressions, compresses the representation, and optimizes item expressiveness by summarizing with more fundamental and contextual key phrases.



Specifically, we crawled reviews for item $i$ from IMDb\footnote{https://www.imdb.com/} and selected the top-$k$ reviews based on helpful votes. Using an LLM, we extracted and summarized common preferences from the reviews and identified keyphrases to optimize item expressiveness. This process condenses the representation, diminishes redundancy, and enhances contextual relevance.
\begin{equation}
    T_{\mathit{r}}^{\mathrm{sum}} = f_{\mathrm{LLM}}(P_{\mathrm{summary}}, T_{\mathrm{m}}, \{r\}_{i=1}^{k}),
\end{equation}
where $r$ denotes individual reviews that have been crawled, and the top-$k$ reviews are inserted into the prompt. The common preferences summary for all the generated reviews is $T_{\mathit{r}}^{\mathrm{sum}}$, which is then processed through an LLM to extract keyphrases.
\begin{equation}
    T_{\mathit{r}}^{\mathrm{key}} = f_{\mathrm{LLM}}(P_{\mathrm{keyphrase}}, T_{\mathit{r}}^{\mathrm{sum}}).
\end{equation}

Further explanation, along with concrete examples of this process, is provided in Appendix~\ref{sec:appendix_prompt}.

\subsection{Preference-aware Learning}
\label{sec:preference_learning}
Existing studies~\cite{pref/crs2021revcore, pref/crs2024ecr} utilize differentiated user preferences to enhance user representation. In contrast, we explicitly represent these preferences separately from the conversation and learn the relationship between them to directly engage the preferences in item scoring.
% Existing studies~\cite{pref/crs2021revcore, pref/crs2024ecr}은 서로 다른 user preference를 구별하여 user representation을 enhance하기 위해 사용한다.
% 반면, 우리는 구별한 preference으로 item scoring에 직접 관여시켜주기 위해, 구별한 user preference를 conversation과 분리하여 표현하고, 이들 간의 관계를 학습한다.
% 또한, user와 preference, item의 관계를 직접적으로 모델링하고 (Section~\ref{sec:matching}), conversation만으로 맞히기 어려운 sample들을 preference를 통해 구분하도록 학습하며 user-preference-item 간 관계를 학습한다 (Section~\ref{sec:training}).

\subsubsection{Preference Modeling}
\label{sec:matching}
\textbf{Representation.} Given the encoding function $f_{\text{Enc}}$ and the dialogue history $T_c$, the vector representation of the dialogue history $c$ is denoted as $\mathbf{h}_c = f_{\text{Enc}} (T_c) \in \mathbb{R}^d$. To be specific, $T_c$ is tokenized and then passed through a text encoder. The final hidden states of all tokens are subsequently mean-pooled, followed by L2 normalization to derive $\mathbf{h}_c$.
% The vector representation of the dialogue history $c$ is denoted as $\mathbf{h}_c = f_{\text{Enc}} (T_c) \in \mathbb{R}^d$. The process of obtaining $\mathbf{h}_c$ through the encoding function $f_{\text{Enc}}$, given the dialogue history $T_c$, proceeds as follows.
\begin{align}
    % h_c = f_\mathrm{Enc}(T_c),\text{where} \\
    [t_1, \dots, t_w] & = \text{Tokenize}(T_c) \\
    [\mathbf{o}_1, \dots, \mathbf{o}_w] & = \text{Enc}([t_1, \dots, t_w]) \\
    \mathbf{h}_c = \frac{\mathbf{o}_c}{\|\mathbf{o}_c\|_2},&~\text{where}~\mathbf{o}_c = \frac{1}{w} \sum_{i=1}^{w} \mathbf{o}_i,
\end{align}
where $\mathbf{o} \in \mathbb{R}^d$ is the contextualized embedding vector, $t$ is the tokenized token and $w$ is the length of tokenized $T_c$.
% \textbf{Version 2}
% \begin{align}
%     h_c & = f_\mathrm{Enc}(T_c) \\
%     & = \text{Norm}(\text{Mean}(\mathrm{Enc}(Tok.(T_c)))).
% \end{align}
% \textbf{Version 3}
% \begin{align}
% [o_1, \dots, o_w] &= \text{Enc}([t_1, \dots, t_w]) \\
%                   &= \text{Enc}(\text{Tokenize}(T_c)) \\
% \mathbf{h}_c &= \frac{\mathbf{o}_c}{\|\mathbf{o}_c\|}, \\
%  & \text{where} \quad \mathbf{o}_c = \frac{1}{w} \sum_{i=1}^{w} \mathbf{o}_i
% \end{align}

Similarly, for $T_{\mathit{l}}^{\mathrm{aug}}$ and $T_{\mathit{d}}^{\mathrm{aug}}$, we obtain the two ambivalent preference representations, $\mathbf{h}_l$ and $\mathbf{h}_d$.
\begin{align}
    \mathbf{h}_l = f_\mathrm{Enc}(T_{\mathit{l}}^{\mathrm{aug}})~\text{and}~\mathbf{h}_d = f_\mathrm{Enc}(T_{\mathit{d}}^{\mathrm{aug}}).
\end{align}

Inspired by previous work~\cite{ret/rs2024blair, data2024AlignLM2IR}, we concatenate item metadata and review information to obtain a review-enhanced item vector representation.
% Inspired by previous work~\cite{ret/rs2024blair, data2024AlignLM2IR}, item의 경우 metadata 정보와 review 정보를 concatenate하여 review-enhanced item vector representation을 구한다.
\begin{align}
    \mathbf{h}_i &= f_\mathrm{Enc}(T_m \oplus T_{\mathit{r}}^{\mathrm{key}} ).
\end{align}

Consequently, we obtain three user-side representations (\ie, $\mathbf{h}_c$, $\mathbf{h}_l$, and $\mathbf{h}_d$) and one item-side representation (\ie, $\mathbf{h}_i$).

% 최종적으로, 우리는 user side representation 3개와 ($\mathbf{h}_c$, $\mathbf{h}_l$, $\mathbf{h}_d$) item side representation 1개 ($\mathbf{h}_i$) 얻는다.



\vspace{0.5mm}
\noindent \textbf{Similarity scoring.}
We linearly aggregate three scores—the similarity between the conversation and item, between like preference and item, and between dislike preference and item—to compute the final score.
The goal is to ensure that the desired item is close to the conversation context and the user's like preference, while being far from the user's dislike preference.
This can be reformulated from Equation~\eqref{overall_scoring} and expressed as follows.
% 우리는 세 가지의 score (conversation와 item, like와 item, 그리고 dislike와 item의 similarity)를 linear하게 aggregate하여 최종 score를 구한다.
% 우리의 목표는 사용자가 원하는 아이템은 대화의 맥락과 사용자의 like preference와는 유사하면서 사용자의 dislike preferene와는 거리가 멀어지게 하는 것이다.
% 이는 Equation~\eqref{overall_scoring}을 reformulate하여 다음과 같이 표현된다.
\begin{align}
S(c, i) &= \text{sim}(\mathbf{h}_c, \mathbf{h}_i) \nonumber \\
        &\quad + \alpha \, \text{sim}(\mathbf{h}_l, \mathbf{h}_i) - \beta \, \text{sim}(\mathbf{h}_d, \mathbf{h}_i),
\end{align}
where $\alpha, \beta \in (0, 1]$ are hyperparameters representing the importance of the user's like and dislike preferences. Empirically, $\alpha$ is set to 0.5, while $\beta$ is adjusted according to the dataset.
% where $\alpha$와 $\beta$는 사용자의 like preference와 dislike preference의 weight를 나타내는 hyperparameter and $\alpha, \beta \in (0, 1]$.

This is a simple yet effective way of reflecting ambivalent preference, requiring no additional parameters.

% 이는 추가로 파라미터를 필요로 하지 않는 간단한 방식이면서 ambivalent한 preference를 반영하는 효과적인 방식이다.

\subsubsection{Training}
\label{sec:training}
% Finally, 우리는 \ours를 학습하는 방법에 대해 설명한다.

\noindent \textbf{Hard negative sampling.}
It is crucial in representation learning because it enhances the model's discriminative ability by focusing on difficult-to-distinguish samples, leading to more efficient learning~\cite{neg2021ANCE,neg2021CLw/Neg}. Additionally, the informativeness of these hard negatives directly impacts the convergence and effectiveness of dense retrieval models.
% The effectiveness of hard negative sampling in representation learning has been highlighted in several previous studies~\cite{neg2021ANCE,neg2021CLw/Neg}. Hard negative sampling은 구분하기 어려운 sample들을 학습하며 모델의 구별 능력을 극대화하고, 더 효율적으로 학습할 수 있게끔 한다.
% The convergence of dense retrieval model training relies on the informativeness of constructed negatives

Our key contribution lies in utilizing hard negative sampling to enhance the representation of user preferences, especially for samples that are challenging to predict based on conversation alone.
Specifically, we first compute the similarity between $\mathbf{h}_c$ and all item embeddings $\mathbf{h}_i$, then apply softmax to convert the similarity scores into a probability distribution. Using this distribution $\{p_{c,i}\}_{i \in I}$, we then sample $k$ negative items, resulting in a set of hard negative samples, further enriching the model's understanding of user preferences.
\begin{align}
    p_{c,i} &= \frac{\exp(\mathrm{sim}(\mathbf{h}_c, \mathbf{h}_i))}{\sum_{j \in \mathcal{I}} \exp((\mathrm{sim}(\mathbf{h}_c, \mathbf{h}_j))} \\
    {\mathcal{I}_c}^- &= \{i_1, i_2, \dots, i_k\} \nonumber \\
    & \sim \text{Multinomial}\left(k, \{p_{c,i}\}_{i \in \mathcal{I}}\right).
\end{align}
%Representation learning에서 hard negative sampling의 효과성은 이전 많은 연구~\cite{neg2021ANCE,neg2021CLw/Neg}에서 highlighted 되었다.
% The key idea of our hard negative sampling은 conversation만으로 맞히기 어려워하는 sample들에 대해 preference까지 사용해서 맞히도록 하며 preference 표현을 enhance하는 것이다.
% 먼저 $h_c$와 전체 아이템의 $h_i$의 유사도를 계산한 후, softmax를 취해서 score을 확률 분포로 변환한다.
% 그 후 확률 분포 $\{p_{u,i}\}_{i \in I}$를 사용해서 $k$개의 negative item을 sampling한다.

\vspace{0.5mm}
\noindent
\textbf{Loss function.}
For training, we utilize the cross-entropy loss following~\cite{ir2020dpr, pref/crs2021revcore, ce2023MARS}.
\begin{equation} \label{eq:training_loss}
    \mathcal{L} = - \log\frac{\text{exp}\left(S \left( c,i^{+}\right) / \tau \right)}{\sum_{i \in {\mathcal{I}_c}^-} {\text{exp}\left( S\left( c,i \right) / \tau\right)}},
\end{equation}
where $i^{+}$ is positive item of $c$, and $\tau$ is hyperparameter to adjust the temperature.

==> body/backup/5_related_work_backup241011.tex <==
% 이런 식으로 다시 작성해볼게요 (내일 오후까진 완성해볼게요 감사합니다)

% 1. CRS 설명, 두 가지 Task 설명
% 2. Traditional CRS 모델 소개 및 한계점 / Preference-aware CRS 모델 언급
% 3. Existing Preference-aware CRS 모델 소개 및 한계점
% 4. 두 가지 Question 던지기
%    4-1. Q1: 사용자가 좋아하고 싫어하는걸 어떻게 알거고, 이걸 어떻게 표현할거임? (how to represent)
%    4-2. Q2: 사용자가 좋아하고 싫어하는 걸 어떻게 item과 align해서 추천할거임? (how to align)
% 5. 제안 방법 소개
%    5-1. A1: 추출하고 증강하고 text로 표현 (semantic, context 키워드 강점)
%    5-2. A2: representation learnining (user <-> positive preference and negative preference <-> item)
%         - retrieval-based CRSs의 이점 언급
% 6. Contribution


% 구성 계획
% Traditional CRS 소개하며, Preference 고려하는 것의 한계와 중요성 언급 후, 아래 카테고리로 전개
% 1. Preference-aware CRS.
% 2. Retrieval-based CRS
% ours와의 차별점을 위 카테고리 각각에 짧게 넣을지, 마지막에 종합적으로 넣을지 고려 중에 있음

\section{Related Work}
\label{sec:related_work}
% KG 사용하는 CRS models
Traditional conversational recommender systems (CRSs) increasingly leverage external information, such as knowledge graphs~\cite{kg/crs2019kbrd, kg/crs2020kgsf, kg/crs2024kascrs, kg/crs2022unicrs, kg/crs2023c2crs} and metadata~\cite{meta/crs2022mese}, to enhance domain knowledge~\cite{survey/crs2021CRSsurvey}. They have utilized additional knowledge bases to support domain-specific entity recognition and expand the system's understanding of world knowledge.
% LLMs 사용하는 CRS models
With the substantial impact of large language models (LLMs) demonstrating exceptional world knowledge, recent studies~\cite{llm/crs2023llmzs, rs2023chatgptgoodrec, llm/crs2024chatcrs, llm/crs2024feedbackcrs} have focused on utilizing LLMs as standalone recommenders.
% LLMs와 KG를 함께 사용하는 CRS models
At the same time, several approaches~\cite{} have been proposed to integrate the strong contextual understanding of LLMs with knowledge graphs to address gaps in domain-specific knowledge. These approaches emphasize leveraging LLMs to infer the most relevant entity relations, while knowledge graphs provide the necessary domain-specific augmentation to enhance the system's overall performance~\cite{llm/crs2021kgensam,llm/crs2024chatcrs}.
% traditional CRS models의 한계점
However, these studies often overlook the fact that users in dialogue may have varied emotions and attitudes toward each entity mentioned. This oversight is significant because it fails to fully capture the complexity of the conversation and, consequently, limits the ability to enhance the user experience.


\noindent
\textbf{Preference-aware CRSs.}
Various studies have focused on improving user preferences at the entity level by considering user emotions using knowledge graphs\cite{pref/crs2021revcore, pref/crs2024ecr}. For instance, RevCore\cite{pref/crs2021revcore} classifies entities extracted from conversations as either positive or negative and then retrieves emotion-related reviews based on this classification, enriching the user's expressive capabilities. In contrast, ECR\cite{pref/crs2024ecr} utilizes LLMs to categorize entities in user utterances into nine fine-grained emotional categories, thereby refining the analysis of user preferences. 그러나, context를 고려하지 않은 모든 entity에 대한 사용자의 선호를 고려하는 것은 사용자의 current demand에 부합하지 않은 irrelevant preference를 고려하게 될 수 있다. 이에 MemoCRS\cite{llm/crs2024memocrs} emphasizes preference continuity by proposing a memory-enhanced approach that considers the user's sequential preferences.
위의 연구들이 사용자의 선호를 다양한 세분성 수준과 context를 고려하고 있지만, 여전히 각각의 연구는 서로 상충되는 선호 정보—즉, positive와 negative—의 존재를 간과하고 있다. 이런 선호 정보를 서로 다르게 고려하지 않는 것은 아이템 추천 시 사용자의 의도를 정확하게 반영하지 못해 결과적으로 suboptimal한 추천 결과를 도출할 수 있다.
% Nevertheless, taking into account user preferences for all entities without considering the context may lead to the incorporation of irrelevant preferences that do not align with the user’s current demands. To address this issue, MemoCRS\cite{llm/crs2024memocrs} underscores the importance of preference continuity by advocating for a memory-enhanced approach that integrates the user’s sequential preferences. Although the studies mentioned previously consider user preferences across various levels of granularity and within different contexts, they consistently neglect the presence of conflicting preference information—specifically, positive and negative aspects. The failure to adequately address these divergent preferences may result in suboptimal recommendation outcomes, as it does not accurately reflect the user's intentions in the recommendation process.

\noindent
\textbf{Retrieval-based CRSs.}
최근 연구에서는 추천 시스템을 아이템 검색 작업으로 재해석하여, 언어 모델의 semantic understanding과 matching 능력을 극대화하려는 시도가 이루어지고 있다~\cite{ret/rs2024blair, data2024AlignLM2IR, ret/crs2023CRSRetbaseline, ret/crs2024nls}. 이를 통해, retriever를 활용하여 CRS task를 개선하는 혁신적인 방법들이 도입되고 있다~\cite{ret/crs2023CRSRetbaseline, ret/crs2024nls}. 특히,~\cite{ret/crs2023CRSRetbaseline}은 대화를 쿼리로, 아이템을 문서로 간주하고, BM25~\cite{bm252021pyserini}와 같은 텍스트 매칭 기법을 사용하여 사용자와 가장 관련성이 높은 아이템을 검색하는 방법을 제안하여 높은 일반화성과 확장성을 지닌다.
또한, 일부 연구에서는 기존의 언어 모델이 아이템 추천 및 검색 작업에 최적화되지 않았다는 점을 지적하며, 제품 임베딩을 위한 사전 학습 접근법~\cite{ret/rs2024blair}이나 아이템 검색을 위한 언어 모델 임베딩 학습용 데이터셋~\cite{data2024AlignLM2IR}을 제안하고 있다.
이러한 Retrieval-based approach는 텍스트로 명시된 사용자의 선호를 반영하는데 효과적인 구조를 제공하지만, 서로 상충되는 선호가 존재하는 CRS에 traditional IR 학습 및 검색 방식을 그대로 적용하는 것은 부적합하다.
% Recent studies reformulate recommendation systems as item retrieval tasks, endeavoring to maximize the semantic understanding and matching capabilities of language models~\cite{ret/rs2024blair, data2024AlignLM2IR, ret/crs2023CRSRetbaseline, ret/crs2024nls}. This shift has led to the introduction of innovative retrieval-based methods designed to enhance the CRS task~\cite{ret/crs2023CRSRetbaseline, ret/crs2024nls}. Specifically,\cite{ret/crs2023CRSRetbaseline} suggests a novel approach by treating dialogues as queries and items as documents, employing text matching techniques such as BM25\cite{bm252021pyserini}, which significantly increases the generalizability and scalability of the retrieval process.
% Additionally, certain studies point out that traditional language models are not ideally optimized for the tasks of item recommendation and retrieval. They advocate for pre-training strategies tailored to product embeddings~\cite{ret/rs2024blair} and the creation of specialized datasets for training language model embeddings dedicated to item retrieval~\cite{data2024AlignLM2IR}.
% Although this retrieval-based approach effectively mirrors users' explicit textual preferences, directly applying traditional Information Retrieval (IR) methodologies in CRS contexts, where conflicting preferences prevail, is deemed unsuitable.

% 본 논문에서는 LLM의 강력한 추론 능력을 활용하여 복잡한 대화에서 사용자의 명시적 선호를 'like'와 'dislike'로 분류하고, recommendation task에 적합하도록 사용자의 잠재적 선호를 추가로 추론한다. 

==> body/backup/5_results_backup241015.tex <==
\section{Results and Analysis}
\input{figures/figures_tex/fig_slm}
\input{tables/tab_zero_shot}
\input{figures/figures_tex/fig_visualization}
\input{figures/figures_tex/fig_case_study}
\label{sec:results}

\subsection{Overall Performance}
Table~\ref{tab:overall_performance} compares \ours~against seven baselines across three datasets.

% 전반적인 성능
\ours achieves state-of-the-art performance, improving Recall@50 and NDCG@50 by an average of 43.87\% and 48.59\%, respectively, over the best competitive baseline. This demonstrates that \ours consistently captures and models user preferences across datasets with diverse characteristics.
% \ours는 3개의 데이터셋에서 Recall@50과 NDCG@50을 best competitive baseline 대비 평균 43.87\%, 48.59\% improve하며 state-of-the-art의 성능을 달성한다. 이것은 \ours가 서로 다른 특징을 가진 데이터셋에서 일관적으로 사용자의 선호를 포착하고 모델링한다는 것을 의미한다.
% sentiment 쓰는 baseline들
사용자의 sentiment를 활용하는 Revcore, ECR과 사용하지 않는 UniCRS를 비교했을 때, \inspired와 \pearl에서는 전자가 더 효과적이나, \pearl에서는 그렇지 않음을 확인할 수 있다.
We assume that \pearl has relatively longer dialogues (refer to Table~\ref{tab
}), which necessitates a more ability to consider the conversational context.
Revcore extracts sentiment at the entity level, and ECR at the utterance level, making it challenging to capture sentiment considering the full context.
% We assume that \pearl의 dialogue가 상대적으로 더 길어서 (Refer to Table \ref{tab:data_statistics}) 대화의 맥락을 고려하는 능력이 더 필요시되기 때문이라고 생각한다.
% Revcore는 entity-level로, ECR은 utterance-level로 sentiment를 도출하여 full context를 고려한 sentiment를 도출하기 어렵다.
하지만 우리는 conversation-level로 sentiment를 도출하고, LLM의 reasoning 능력으로 표면적인 선호뿐만 아니라 potential한 선호까지 고려하기 때문에 대화 흐름 내에서 더 사용자의 전반적인 선호도를 명확하게 파악할 수 있음
% 가장 가까운 baseline과의 비교
또한, \ours~outperform ECR~\cite{pref/crs2024ecr} that 사용자의 sentiment를 사용하여 user representation을 enhance하는.
이는 preference를 explicit하게 고려하는 것이 user preference modeling을 효과적으로 나타내는 방법임을 의미한다.


\subsection{Further Analysis}
\subsubsection{Performance by Model Size}
이 section에서는 \ours를 다양한 모델 크기의 backbone에 적용해본 후 결과를 비교한다.
Figure \ref{fig:slm}
이러한 실험 결과를 기반으로 우리는 크게 두 observation을 얻었다.
(i) 모델 크기가 커질 수록 성능이 올라간다. Model size가 BERT-base (110M), FlanT5-XL (1.5B), NV-Embed (7B)으로 커질수록 성능이 올라간다.
(ii) 같은 backbone을 공유하는 DPR과 비교했을 때, \ours가 NDCG@50에서 39\%의 gain을 보여준다.
이러한 결과는 \ours가 scalability가 뛰어나며, 모델 크기에 상관없이 적용될 수 있는 범용적이고 effective한 framework임을 드러낸다.
% 또한 비슷한 모델 크기에서 \ours~(BERT)가 DPR~(BERT)와 ECR과 비슷하거나 더 높은 성능을 보인다.


\subsubsection{Zero-shot Performance}
Table \ref{tab:lm_zero_shot}는 sparse retriever과 두 서로 다른 크기의 dense retriever 위에서 \ours의 zero-shot performance를 evaluate한다.
이때 item textual representation으로는 $T_m$과 ${T_r}^{\mathrm{key}}$를 concat하여 사용하였다.
As reported in Table \ref{tab:lm_zero_shot}, \ours는 backbone에 무관하게 크게 성능을 향상시킨다, achieving 37\% performance gain on average. 
이는 두 가지를 의미하는데요.
(i) 우리가 추출한 user preference가 다양한 retriever 구조와 size에서도 effective하다.
(ii) Similarity scoring이 학습 없이도 conv와 like, dislike 그리고 item 간 관계를 효과적으로 모델링한다.

\subsubsection{Ablation Study}
\input{tables/tab_ablation}
\ours의 각 component가 성능에 어떤 영향을 미치는지 알기 위해 우리는 \inspired에서 ablation study를 진행하였다.
The results are show in Table~\ref{tab:Ablation study}.

우리는 먼저 preference expansion의 유효성에 대해 검증한다.
$L, D, R$은 각각 $T_{\mathit{l}}^{\mathrm{aug}}, T_{\mathit{d}}^{\mathrm{aug}}, T_{\mathit{r}}^{\mathrm{key}}$를 의미한다. 이때 \emph{w/o $L$}은 train 및 inference 시에 $T_{\mathit{l}}^{\mathrm{aug}}$를 사용하지 않았다는 것을 의미한다.
이때 증강된 세 preference가 모두 성능에 기여하며, 특히 낮은 cutoff에서 성능 향상에 효과적이다.
이는 preference를 사용함으로써 subtle preference를 구분할 수 있기 때문이다.

% Variant \emph{w/o $L, D$}는 train 및 inference 시에 사용자의 like/dislike preference $T_{\mathit{l}}^{\mathrm{aug}}, T_{\mathit{d}}^{\mathrm{aug}}$를 사용하지 않고 dialogue history $T_c$만 사용하는 variant이며, \emph{w/o $K$}는 train 및 inference 시에 아이템의 review summary $T_\mathit{keyphrase}$는 사용하지 않고 metadata $T_m$만 사용하는 variant이다. \emph{w/o $L, D, K$}는 $T_{\mathit{l}}^{\mathrm{aug}}, T_{\mathit{d}}^{\mathrm{aug}}, T_{\mathit{keyphrase}}$를 모두 사용하지 않는 variant이다. 
또한 we investigate the effectiveness of user의 potential preference를 증강하는 것. \emph{w/o $Aug.$}는 current preference extraction만 거친 $T_{\mathit{l}}^{\mathrm{ext}}, T_{\mathit{d}}^{\mathrm{ext}}$를 사용자의 positive and negative preference로 사용한다. Compared to Ours, the result 선호를 추출하는 것뿐만 아니라 그 안에 내재된 preference를 파악하는 것이 중요함을 highlight한다.
We then explore the effects of preference-aware learning.
\emph{w/o Neg.}는 hard negative를 사용하지 않고 in-batch negative를 사용한 variant이고, \emph{w/o PL}은 preference modeling과 hard negative를 사용하지 않은 variant이다. \emph{w/o PL}의 경우 $T_c, T_{\mathit{l}}^{\mathrm{ext}}, T_{\mathit{d}}^{\mathrm{ext}}$를 concat하여 하나의 user text represenation을 만든 후 CL loss를 사용하여 학습했다. Compared to \ours, the result indicates that preference-aware learning effectively learn the relationship between conversation, preferences and item.

\subsubsection{Visualization}
Figure~\ref{fig:visualization}는
\subsection{Case Study}
Figure~\ref{fig:case_study}는 \pearl 데이터셋에서 \ours가 Recall@1로 정확히 맞춘 샘플에서, like와 dislike가 가장 바람직하게 모델링된 경우를 보여준다. 가장 이상적인 형태는 user의 dislike가 item의 실제 dislike와 겹치지 않고, dislike와 반대되는 개념이 like에 포함되는 것이다. 반면, like의 경우는 user의 preference가 item의 like 정보와 유사하게 대응해야 한다.
Figure~\ref{fig:case_study}에서 같은 색으로 하이라이팅된 부분은 동일한 개념에 속하는 키프레이즈를 의미한다. 그림에서 볼 수 있듯이, user의 like preference는 모두 item의 like preference와 정확히 대응하고 있음을 확인할 수 있다. 또한, user의 dislike preference인 "predictable plots that lack depth"는 item의 like에 해당하는 'tension and suspenseful storyline'과 반대되는 개념으로 대응된다.
이를 통해, \ours가 제안한 증강 방법을 활용하면 기존 주어진 dialogue history만으로는 예측하기 어려운 user preference를 보다 효과적으로 예측할 수 있음을 알 수 있다. 제안된 방식은 ambivalent한 선호도를 고려해 user preference를 더욱 세밀하게 구분하여 학습하는 데 효과적임을 보여준다.

==> body/backup/5_results_backup2410152330.tex <==
\section{Results and Analysis}
\input{figures/figures_tex/fig_slm}
\input{tables/tab_zero_shot}
\input{figures/figures_tex/fig_visualization}
\input{figures/figures_tex/fig_case_study}
\label{sec:results}

\subsection{Overall Performance}
Table~\ref{tab:overall_performance} compares \ours~against seven baselines across three datasets.
% 전반적인 성능
\ours~achieves state-of-the-art performance, improving Recall@50 and NDCG@50 by an average of 43.87\% and 48.59\%, respectively, over the best competitive baseline. This demonstrates that it consistently captures and models user preferences across datasets with diverse characteristics.
% \ours는 3개의 데이터셋에서 Recall@50과 NDCG@50을 best competitive baseline 대비 평균 43.87\%, 48.59\% improve하며 state-of-the-art의 성능을 달성한다. 이것은 \ours가 서로 다른 특징을 가진 데이터셋에서 일관적으로 사용자의 선호를 포착하고 모델링한다는 것을 의미한다.
% 가장 가까운 baseline과의 비교
Additionally, \ours~outperforms ECR~\cite{pref/crs2024ecr}, which enhances user representation by using sentiment. This indicates that explicitly learning the relationships between preferences and users/items is more effective for user preference modeling.
% 또한, \ours~outperform ECR~\cite{pref/crs2024ecr} that 사용자의 sentiment를 사용하여 user representation을 enhance하는. 이는 preference와 user/item 간의 관계를 explicitly 학습하는 것이 user preference modeling에 효과적임을 나타한다.

% sentiment 쓰는 baseline들
Revcore and ECR, which utilize user sentiment, are effective compared to UniCRS in \inspired~but not in \pearl.
We assume that \pearl~has relatively longer dialogues (Refer to Table~\ref{tab:data_statistics}), which necessitates a greater ability to consider the conversational context.
Revcore extracts sentiment at the entity level, and ECR at the utterance level, making it challenging to capture sentiment considering the full context.
% We assume that \pearl의 dialogue가 상대적으로 더 길어서 (Refer to Table \ref{tab:data_statistics}) 대화의 맥락을 고려하는 능력이 더 필요시되기 때문이라고 생각한다.
% Revcore는 entity-level로, ECR은 utterance-level로 sentiment를 도출하여 full context를 고려한 sentiment를 도출하기 어렵다.
However, \ours~identifies user sentiment at the conversation-level utilizing the reasoning capabilities of LLM, thereby achieving a more comprehensive understanding of user preference within the dialogue.
% 하지만 우리는 LLM의 reasoning 능력 기반으로 conversation-level로 sentiment를 파악하기 때문에 대화 흐름 내에서 더 사용자의 전반적인 선호도를 명확하게 파악할 수 있음

\subsection{Further Analysis}
\subsubsection{Performance by Model Size}
Figure~\ref{fig:slm} presents the performance of \ours~on an LLM backbone with different model sizes, and we have two observations as follows.
% Figure~\ref{fig:slm}은 \ours를 다양한 모델 크기의 backbone에 따른 성능을 보여주며, 우리는 두 observation을 얻었다.
(i) The performance increases as the model size increases to BERT-base (110M), FlanT5-XL (1.5B), NV-Embed (7B). 이것은 큰 모델일수록 텍스트의 복잡한 의미적 관계를 더 잘 포착할 수 있고, \ours가 dense retriever 구조를 사용하여 take full advantage of PLM이기 때문.
(ii) Compared to DPR, which shares the same backbone, \ours shows a 39\% gain in NDCG@50.
These results show that \ours~is a highly scalable, universal and effective framework that can be applied to any model size.
% (i) LLM 모델 크기가 커질 수록 성능이 올라간다. Model size가 BERT-base (110M), FlanT5-XL (1.5B), NV-Embed (7B)으로 커질수록 성능이 올라간다.
% (ii) 같은 backbone을 공유하는 DPR과 비교했을 때, \ours가 NDCG@50에서 39\%의 gain을 보여준다.
% 이러한 결과는 \ours가 scalability가 뛰어나며, 모델 크기에 상관없이 적용될 수 있는 범용적이고 effective한 framework임을 드러낸다.
% 또한 비슷한 모델 크기에서 \ours~(BERT)가 DPR~(BERT)와 ECR과 비슷하거나 더 높은 성능을 보인다.


\subsubsection{Zero-shot Performance}
% Table~\ref{tab:lm_zero_shot} evaluates the zero-shot performance of \ours~on a sparse retriever and two dense retrievers of different sizes.
% 이때 ambivalent preference의 textual representation 대신 $T_m$과 ${T_r}^{\mathrm{key}}$를 concat하여 사용하였다.
% \ours~significantly improves performance independent of the backbone, achieving a 37\% performance gain on average.
% 이는 두 가지를 의미한다.
% (i) 우리가 추출한 user preference가 다양한 retriever 구조와 size에서도 effective하다.
% (ii) Similarity scoring이 학습 없이도 conv와 like, dislike 그리고 item 간 관계를 효과적으로 모델링한다.
To investigate the effectiveness of ambivalent preference expansion, we caculate the zero-shot performance of \ours~using a sparse retriever and two dense retrievers of varying sizes. For the item-side textual representation we concatenated $T_m$ with ${T_r}^{\mathrm{key}}$.
\ours~significantly improves performance across different backbones, demonstrating a 37\% average gain in the zero-shot setting.
The results confirm that ambivalent preference expansion effectively improves recommendation performance by inferring potential user preferences. More detailed ablation for ambivalent preferences of the user-side can be found in Appendix~\ref{sec:appendix_zero_shot_ablation}.

% Table~\ref{tab:lm_zero_shot}에서, \ours~significantly improves performance independent of the backbone, achieving a 37\% performance gain on average in zero-shot setting. 이때 ambivalent preference의 textual representation 대신 $T_m$과 ${T_r}^{\mathrm{key}}$를 concat하여 사용하였다. 
% We evaluate the zero-shot performance of \ours~on a sparse retriever and two dense retrievers of different sizes. 실험 결과는 우리가 증강한 potential user preference가 추천 성능을 개선하는 recommendation-tailored augmentation approach임을 입증한다. like/dislike의 다양한 ablation setting에서의 결과는 Table~\ref{tab:zs_ablation}에서 확인할 수 있다.

\subsubsection{Ablation Study}
\input{tables/tab_ablation}
To understand the impact of each component of \ours~on performance, we conducted an ablation study on \inspired, as shown in Table~\ref{tab:Ablation study}.
% \ours의 각 component가 성능에 어떤 영향을 미치는지 알기 위해 우리는 \inspired에서 ablation study를 진행하였다, are shown in Table~\ref{tab:Ablation study}.

First, we validate the effectiveness of preference expansion.
Let $L$, $D$ and $R$ denote $T_{\mathit{l}}^{\mathrm{aug}}$, $T_{\mathit{d}}^{\mathrm{aug}}$, and $T_{\mathit{r}}^{\mathrm{key}}$, respectively. Here, \emph{w/o $L$} means that $T_{\mathit{l}}^{\mathrm{aug}}$ was not used in both train and inference.
In this case, all three augmented preferences contribute to performance, especially at low cutoffs.
This is because the use of preference allows us to distinguish subtle preferences.

% 우리는 먼저 preference expansion의 유효성에 대해 검증한다.
% $L, D, R$은 각각 $T_{\mathit{l}}^{\mathrm{aug}}, T_{\mathit{d}}^{\mathrm{aug}}, T_{\mathit{r}}^{\mathrm{key}}$를 의미한다. 이때 \emph{w/o $L$}은 train 및 inference 시에 $T_{\mathit{l}}^{\mathrm{aug}}$를 사용하지 않았다는 것을 의미한다.
% 이때 증강된 세 preference가 모두 성능에 기여하며, 특히 낮은 cutoff에서 성능 향상에 효과적이다.
% 이는 preference를 사용함으로써 subtle preference를 구분할 수 있기 때문이다.
% Variant \emph{w/o $L, D$}는 train 및 inference 시에 사용자의 like/dislike preference $T_{\mathit{l}}^{\mathrm{aug}}, T_{\mathit{d}}^{\mathrm{aug}}$를 사용하지 않고 dialogue history $T_c$만 사용하는 variant이며, \emph{w/o $K$}는 train 및 inference 시에 아이템의 review summary $T_\mathit{keyphrase}$는 사용하지 않고 metadata $T_m$만 사용하는 variant이다. \emph{w/o $L, D, K$}는 $T_{\mathit{l}}^{\mathrm{aug}}, T_{\mathit{d}}^{\mathrm{aug}}, T_{\mathit{keyphrase}}$를 모두 사용하지 않는 variant이다. 
We also investigate the effect of augmenting user's potential preferences.
We use $T_{\mathit{l}}^{\mathrm{ext}}$, $T_{\mathit{d}}^{\mathrm{ext}}$ as the user's positive and negative preferences with only current preference extraction.
Compared to \ours, the result emphasizes the importance of understanding the underlying preference in the dialogue.
% 또한 we investigate the effectiveness of user의 potential preference를 증강하는 것. \emph{w/o $Aug.$}는 current preference extraction만 거친 $T_{\mathit{l}}^{\mathrm{ext}}, T_{\mathit{d}}^{\mathrm{ext}}$를 사용자의 positive and negative preference로 사용한다. Compared to \ours, the result 선호를 추출하는 것뿐만 아니라 그 안에 내재된 preference를 파악하는 것이 중요함을 highlight한다.
Finally, we explore the effects of preference-aware learning.
\emph{w/o Neg.} is a variant that uses in-batch negative instead of hard negative, and \emph{w/o PL} is a variant without preference modeling and hard negative, which utilize single user representation by concatenating $T_c, T_{\mathit{l}}^{\mathrm{ext}}, T_{\mathit{d}}^{\mathrm{ext}}$.
Compared to \ours, the result indicates that preference-aware learning effectively learns the relationship between conversation, preferences, and items.

\input{figures/figures_tex/fig_case_study}
\subsection{Case Study}
% Figure~\ref{fig:case_study}는 \pearl에서 \ours가 like와 dislike가 Recall@1로 정확히 맞춘 샘플에서, like와 dislike가 가장 바람직하게 모델링된 경우를 보여준다.
% 우리는 제안 방법의 효과성을 입증하기 위해 case study를 진행하였다. Figure~\ref{fig:case_study}에서 같은 색으로 하이라이팅된 부분은 동일한 개념에 속하는 키프레이즈를 의미한다.
% 그림에서 볼 수 있듯이, user의 like preference는 모두 item의 like preference와 정확히 대응하고 있음을 확인할 수 있다. 또한, user의 dislike preference인 ``\emph{predictable plots that lack depth}''는 item의 like에 해당하는 ``\emph{tension and suspenseful storyline}''과 반대되는 개념으로 대응된다.
% 가장 이상적인 형태는 user의 dislike가 item의 실제 dislike와 겹치지 않고, dislike와 반대되는 개념이 like에 포함되는 것이다. 반면, like의 경우는 user의 preference가 item의 like 정보와 유사하게 대응해야 한다.
% 이를 통해, \ours가 제안한 증강 방법을 활용하면 기존 주어진 dialogue history만으로는 예측하기 어려운 user preference를 보다 효과적으로 예측할 수 있음을 알 수 있다.
% To further explain \ours, we conducted a detailed case study.
% This analysis illustrates how our approach captures user preferences and enhances prediction accuracy, even when user preferences are not immediately apparent from the dialogue history explicitly.

Figure~\ref{fig:case_study}(a) shows a case study of the user's dialogue, the augmented preferences, and the ground truth item from \pearl.
The highlighted phrases in the same color represent key phrases that belong to the same concept and are related to the ground-truth item. 
In particular, the blue, teal, and orange preferences are newly augmented through ambivalent preference expansion.
% User side Expansion
Especially, \ours~effectively inferred the user's preference for thriller and drama genres based on the dialogue.
This demonstrates that by leveraging the augmentation method proposed by \ours, it is possible to more effectively predict user preferences that are difficult to infer solely from the given dialogue history.
% Item side expansion
Also, it can be observed that the user's ambivalent preferences align with the item’s review summary. This indicates that the review summary successfully bridges the gap between the preferences expressed in the user conversation and the item itself.
% Explainability
Additionally, \ours's ambivalent preference expansion serves as a rationale for the recommendation results, thereby providing explainability.

% As shown in the figure, we can observe how augmented preferences match the item's preferences. In particular, the user's dislike preference, \textit{"predictable plots that lack depth,"} corresponds to the opposite concept of the item's like preference, \textit{"tension and suspenseful storyline."}
% 증강된 preference가 어떻게 도움이 되었는지 추가
% 또한, 대화 내의 사용자 preferences들을 기반으로 대화에 언급되지 않은 preference (\eg, predictable plots that lack depth) 등이 효과적으로 추출되고, 이러한 정보가 item의 정보와 matching되는 것을 확인할 수 있다.

% The ideal scenario is where the user's dislikes do not overlap with the item's actual dislikes, and the opposing concept of their dislikes is included in the item's likes. On the other hand, for likes, the user's preferences should closely align with the item's like information.
% To illustrate how \ours~utilize preference, 우리는 Figure~\ref{fig:visualization}에 \pearl에서의 예시를 t-SNE를 사용하여 시각화하였다.
% 예제에서 보이듯이, conversation만 사용했을 때는 like preference보다 dislike preference에 가까운 item이 선택될 수 있다(\eg 예시 넣을 예정).
% 하지만 \ours는 like와 dislike preference를 explicitly 고려하며 user, item과의 관계를 모델링해 사용자의 선호를 올바르게 추출해낼 수 있었다.
We then visualized the same example using t-SNE in Figure~\ref{fig:case_study}(b), to illustrate how \ours~utilizes preference. As shown in the example, sub-optimal may be selected when only the conversation is used. However, since \ours~explicitly considers both like and dislike preferences and models the relationship between the user and the item, it successfully recommended the right item.
